Accelerating Energy-Efficient Federated Learning in Cell-Free Networks with Adaptive Quantization

Federated Learning (FL) enables clients to share learning parameters instead of local data, reducing communication overhead. Traditional wireless networks face latency challenges with FL. In contrast, Cell-Free Massive MIMO (CFmMIMO) can serve multiple clients on shared resources, boosting spectral efficiency and reducing latency for large-scale FL. However, clients' communication resource limitations can hinder the completion of the FL training. To address this challenge, we propose an energy-efficient, low-latency FL framework featuring optimized uplink power allocation for seamless client-server collaboration. Our framework employs an adaptive quantization scheme, dynamically adjusting bit allocation for local gradient updates to reduce communication costs. We formulate a joint optimization problem covering FL model updates, local iterations, and power allocation, solved using sequential quadratic programming (SQP) to balance energy and latency. Additionally, clients use the AdaDelta method for local FL model updates, enhancing local model convergence compared to standard SGD, and we provide a comprehensive analysis of FL convergence with AdaDelta local updates. Numerical results show that, within the same energy and latency budgets, our power allocation scheme outperforms the Dinkelbach and max-sum rate methods by increasing the test accuracy up to $7$\% and $19$\%, respectively. Moreover, for the three power allocation methods, our proposed quantization scheme outperforms AQUILA and LAQ by increasing test accuracy by up to $36$\% and $35$\%, respectively.

==> MetaFiles/PackagesResponseLetter.tex <==
\usepackage{dsfont}
\usepackage{graphicx}
%\usepackage[scanall]{psfrag}
\usepackage{amsfonts}
\usepackage{amssymb}
\usepackage{fancyhdr}
\usepackage{url}
\usepackage{lipsum}
\usepackage{psfrag}
%\usepackage{subfig}
\usepackage{mathrsfs}
\usepackage{dsfont}
\usepackage{subfigure}
\usepackage{epsfig}
\usepackage{xspace}
\usepackage{times}
\usepackage[innercaption]{sidecap}
\usepackage{bm}
\usepackage{url}
\usepackage{color}
\usepackage{xcolor}
\usepackage{lastpage}
\usepackage{fancyhdr}
\usepackage{bbm}
\usepackage{hhline}
\usepackage{multirow}

\usepackage{tikz}
\usetikzlibrary{arrows,decorations.pathmorphing,backgrounds,fit,petri,positioning,matrix}
\usetikzlibrary{shapes,arrows}
\usepackage{multirow}
\newcommand{\addb}[1]{{{\color{blue!60!white}#1}}}
\newcommand{\addr}[1]{{{\color{red!60!black}#1}}}
\usepackage{caption}
\usepackage{centernot}
\usepackage{cite}
\usepackage{amsfonts}
\usepackage{gensymb}

\usepackage{times} % assumes new font selection scheme installed
\usepackage{amsmath} % assumes amsmath package installed
\usepackage{amssymb}  % assumes amsmath package installed
\usepackage{mathrsfs}
\usepackage{array}
\usepackage{algorithm}
\usepackage{algorithmic}
\usepackage{changepage}
\usepackage{soul}

\def\Red#1{\textcolor{red}{#1}}
%\def\Blue#1{\textcolor{blue}{#1}}
\def\Blue#1{\color{blue!70!black}{#1}}
\def\Blak#1{\color{blue!0!black}{#1}}
\def\nota#1{\marginpar{\bf\tiny#1}}
\def\1{\,\mathds{1}\,}

%\newcommand{\ssum}[1]{\displaystyle\mathop{ \textstyle{\sum}}_{#1}}

%\input{acm_macros}


%\newtheorem{theorem}{Theorem}[section]
%\newtheorem{corollary}[theorem]{Corollary}
%\newtheorem{lemma}[theorem]{Lemma}
%\newtheorem{proposition}[theorem]{Proposition}
%\newtheorem{definition}[theorem]{Definition}
%\newtheorem{remark}[theorem]{Remark}
%\numberwithin{equation}{section}

%%%%%%% Page style definition %%%%%%%
\oddsidemargin 0.0cm \evensidemargin 0.0cm \textwidth 16.5cm
\headheight 0cm \topmargin 0.1cm \textheight 22cm

%\pagestyle{fancy} \fancyhf{} \fancyhead[C]{\slshape\sffamily
%Response letter} \fancyfoot[C]{~\thepage~}
\pagestyle{fancy}
\chead{\small Response letter}  %\rhead{\rightmark}
\cfoot{\small \thepage\ of \pageref{LastPage}}

\renewcommand{\headrulewidth}{0.5pt}
\renewcommand{\footrulewidth}{0pt}

\fancypagestyle{plain}{%
    \fancyhf{}
    \renewcommand{\headrulewidth}{0pt}
    \renewcommand{\footrulewidth}{0pt}
}


%% Enviroments for review and author comments:
%\newenvironment{reviewer}{\vspace{0.5cm}\it \noindent\ignorespaces}{\vspace{0.5cm}}
\newenvironment{reviewer}{\vspace{0.5cm}\it \Blue \noindent\ignorespaces}{\vspace{0.2cm}}
\newenvironment{authors}{\rm\Blak\noindent\ignorespaces}{\vspace{0.0cm}}
\linespread{1.5}

\renewcommand{\IEEEQED}{\IEEEQEDopen}

%%%%%%%
\usepackage{algorithm2e}
\SetAlFnt{\small}
\SetAlCapFnt{\large}
\SetAlCapNameFnt{\large}
\usepackage{algorithmic}
\algsetup{linenosize=\tiny}
%%%%%

==> MetaFiles/acronyms.tex <==
%\chapter*{Acronyms}
%\renewcommand{\titulonome}{Acronyms}%
%\renewcommand{\prepbynome}{UFC.33 Team}%

%\begin{singlespace}
\begin{acronym}%[LTE-Advanced]%\addtolength{\itemsep}{-0.5\baselineskip}
  \acro{2G}{Second Generation}
  \acro{3G}{3$^\text{rd}$~Generation}
  \acro{3GPP}{3$^\text{rd}$~Generation Partnership Project}
  \acro{4G}{4$^\text{th}$~Generation}
  \acro{5G}{5$^\text{th}$~Generation}
  \acro{AA}{Antenna Array}
  \acro{AC}{Admission Control}
  \acro{AD}{Attack-Decay}
  \acro{ADSL}{Asymmetric Digital Subscriber Line}
	\acro{AHW}{Alternate Hop-and-Wait}
  \acro{AMC}{Adaptive Modulation and Coding}
	\acro{AP}{Access Point}
  \acro{APA}{Adaptive Power Allocation}
  \acro{ARMA}{Autoregressive Moving Average}
  \acro{ATES}{Adaptive Throughput-based Efficiency-Satisfaction Trade-Off}
  \acro{AWGN}{additive white Gaussian noise}
  \acro{BB}{Branch and Bound}
  \acro{BCD}{block-coordinate descent}
  \acro{BD}{block-diagonalization}
  \acro{BER}{Bit Error Rate}
  \acro{BF}{Best Fit}
  \acro{BLER}{BLock Error Rate}
  \acro{BPC}{Binary power control}
  \acro{BPSK}{Binary Phase-Shift Keying}
  \acro{BPA}{Best \ac{PDPR} Algorithm}
  \acro{BRA}{Balanced Random Allocation}
  \acro{BS}{base station}
  \acro{CAP}{Combinatorial Allocation Problem}
  \acro{CAPEX}{Capital Expenditure}
  \acro{CBF}{Coordinated Beamforming}
  \acro{CBR}{Constant Bit Rate}
  \acro{CBS}{Class Based Scheduling}
  \acro{CC}{Congestion Control}
  \acro{CDF}{Cumulative Distribution Function}
  \acro{CDMA}{Code-Division Multiple Access}
  \acro{CI}{coherence interval}
  \acro{CL}{Closed Loop}
  \acro{CLPC}{Closed Loop Power Control}
  \acro{CNR}{Channel-to-Noise Ratio}
  \acro{CPA}{Cellular Protection Algorithm}
  \acro{CPICH}{Common Pilot Channel}
  \acro{CoMP}{Coordinated Multi-Point}
  \acro{CQI}{Channel Quality Indicator}
  \acro{CRM}{Constrained Rate Maximization}
	\acro{CRN}{Cognitive Radio Network}
  \acro{CS}{Coordinated Scheduling}
  \acro{CSI}{channel state information}
  \acro{CSIR}{channel state information at the receiver}
  \acro{CSIT}{channel state information at the transmitter}
  \acro{CUE}{cellular user equipment}
  \acro{D2D}{device-to-device}
  \acro{DCA}{Dynamic Channel Allocation}
  \acro{DE}{Differential Evolution}
  \acro{DFT}{Discrete Fourier Transform}
%  \acro{DIST}{Distance-based Grouping}
  \acro{DIST}{Distance}
  \acro{DL}{downlink}
  \acro{DMA}{Double Moving Average}
	\acro{DMRS}{Demodulation Reference Signal}
  \acro{D2DM}{D2D Mode}
  \acro{DMS}{D2D Mode Selection}
  \acro{DPC}{Dirty Paper Coding}
  \acro{DRA}{Dynamic Resource Assignment}
  \acro{DSA}{Dynamic Spectrum Access}
  \acro{DSM}{Delay-based Satisfaction Maximization}
  \acro{ECC}{Electronic Communications Committee}
  \acro{EFLC}{Error Feedback Based Load Control}
  \acro{EI}{Efficiency Indicator}
  \acro{eNB}{Evolved Node B}
  \acro{EPA}{Equal Power Allocation}
  \acro{EPC}{Evolved Packet Core}
  \acro{EPS}{Evolved Packet System}
  \acro{E-UTRAN}{Evolved Universal Terrestrial Radio Access Network}
  \acro{ES}{Exhaustive Search}
  \acro{FDD}{frequency division duplexing}
  \acro{FDM}{Frequency Division Multiplexing}
  \acro{FER}{Frame Erasure Rate}
  \acro{FF}{Fast Fading}
  \acro{FSB}{Fixed Switched Beamforming}
  \acro{FST}{Fixed SNR Target}
  \acro{FTP}{File Transfer Protocol}
  \acro{GA}{Genetic Algorithm}
  \acro{GBR}{Guaranteed Bit Rate}
  \acro{GLR}{Gain to Leakage Ratio}
  \acro{GOS}{Generated Orthogonal Sequence}
  \acro{GPL}{GNU General Public License}
  \acro{GRP}{Grouping}
  \acro{HARQ}{Hybrid Automatic Repeat Request}
  \acro{HMS}{Harmonic Mode Selection}
  \acro{HOL}{Head Of Line}
  \acro{HSDPA}{High-Speed Downlink Packet Access}
  \acro{HSPA}{High Speed Packet Access}
  \acro{HTTP}{HyperText Transfer Protocol}
  \acro{ICMP}{Internet Control Message Protocol}
  \acro{ICI}{Intercell Interference}
  \acro{ID}{Identification}
  \acro{IETF}{Internet Engineering Task Force}
  \acro{ILP}{Integer Linear Program}
  \acro{JRAPAP}{Joint RB Assignment and Power Allocation Problem}
  \acro{UID}{Unique Identification}
  \acro{IID}{Independent and Identically Distributed}
  \acro{IIR}{Infinite Impulse Response}
  \acro{ILP}{Integer Linear Problem}
  \acro{IMT}{International Mobile Telecommunications}
  \acro{INV}{Inverted Norm-based Grouping}
	\acro{IoT}{Internet of Things}
  \acro{IP}{Internet Protocol}
  \acro{IPv6}{Internet Protocol Version 6}
  \acro{ISD}{Inter-Site Distance}
  \acro{ISI}{Inter Symbol Interference}
  \acro{ITU}{International Telecommunication Union}
  \acro{JOAS}{Joint Opportunistic Assignment and Scheduling}
  \acro{JOS}{Joint Opportunistic Scheduling}
  \acro{JP}{Joint Processing}
	\acro{JS}{Jump-Stay}
  \acro{KKT}{Karush-Kuhn-Tucker}
  \acro{L3}{Layer-3}
  \acro{LAC}{Link Admission Control}
  \acro{LA}{Link Adaptation}
  \acro{LC}{Load Control}
  \acro{LOS}{Line of Sight}
  \acro{LP}{Linear Programming}
  \acro{LS}{least squares}
  \acro{LTE}{Long Term Evolution}
  \acro{LTE-A}{LTE-Advanced}
  \acro{LTE-Advanced}{Long Term Evolution Advanced}
  \acro{M2M}{Machine-to-Machine}
  \acro{MAB}{multi-armed bandit}
  \acro{MAC}{medium access control}
  \acro{MANET}{Mobile Ad hoc Network}
  \acro{MC}{Modular Clock}
  \acro{MCS}{Modulation and Coding Scheme}
  \acro{MDB}{Measured Delay Based}
  \acro{MDI}{Minimum D2D Interference}
  \acro{MF}{Matched Filter}
  \acro{MG}{Maximum Gain}
  \acro{MH}{Multi-Hop}
  \acro{MIMO}{multiple input multiple output}
  \acro{MINLP}{Mixed Integer Nonlinear Programming}
  \acro{MIP}{Mixed Integer Programming}
  \acro{MISO}{Multiple Input Single Output}
  \acro{MLWDF}{Modified Largest Weighted Delay First}
  \acro{MME}{Mobility Management Entity}
  \acro{MMSE}{minimum mean squared error}
  \acro{MOS}{Mean Opinion Score}
  \acro{MPF}{Multicarrier Proportional Fair}
  \acro{MRA}{Maximum Rate Allocation}
  \acro{MR}{Maximum Rate}
  \acro{MRC}{Maximum Ratio Combining}
  \acro{MRT}{Maximum Ratio Transmission}
  \acro{MRUS}{Maximum Rate with User Satisfaction}
  \acro{MS}{mobile station}
  \acro{MSE}{mean squared error}
  \acro{MSI}{Multi-Stream Interference}
  \acro{MTC}{Machine-Type Communication}
  \acro{MTSI}{Multimedia Telephony Services over IMS}
  \acro{MTSM}{Modified Throughput-based Satisfaction Maximization}
  \acro{MU-MIMO}{multiuser multiple input multiple output}
  \acro{MU}{multi-user}
  \acro{NAS}{Non-Access Stratum}
  \acro{NB}{Node B}
  \acro{NE}{Nash equilibrium}
	\acro{NCL}{Neighbor Cell List}
  \acro{NLP}{Nonlinear Programming}
  \acro{NLOS}{Non-Line of Sight}
  \acro{NMSE}{Normalized Mean Square Error}
  \acro{NORM}{Normalized Projection-based Grouping}
  \acro{NP}{Non-Polynomial Time}
  \acro{NRT}{Non-Real Time}
  \acro{NSPS}{National Security and Public Safety Services}
  \acro{O2I}{Outdoor to Indoor}
  \acro{OFDMA}{orthogonal frequency division multiple access}
  \acro{OFDM}{orthogonal frequency division multiplexing}
  \acro{OFPC}{Open Loop with Fractional Path Loss Compensation}
	\acro{O2I}{Outdoor-to-Indoor}
  \acro{OL}{Open Loop}
  \acro{OLPC}{Open-Loop Power Control}
  \acro{OL-PC}{Open-Loop Power Control}
  \acro{OPEX}{Operational Expenditure}
  \acro{ORB}{Orthogonal Random Beamforming}
  \acro{JO-PF}{Joint Opportunistic Proportional Fair}
  \acro{OSI}{Open Systems Interconnection}
  \acro{PAIR}{D2D Pair Gain-based Grouping}
  \acro{PAPR}{Peak-to-Average Power Ratio}
  \acro{P2P}{Peer-to-Peer}
  \acro{PC}{Power Control}
  \acro{PCI}{Physical Cell ID}
  \acro{PDF}{Probability Density Function}
  \acro{PDPR}{pilot-to-data power ratio}
  \acro{PER}{Packet Error Rate}
  \acro{PF}{Proportional Fair}
  \acro{P-GW}{Packet Data Network Gateway}
  \acro{PL}{Pathloss}
  \acro{PPR}{pilot power ratio}
  \acro{PRB}{Physical Resource Block}
  \acro{PROJ}{Projection-based Grouping}
  \acro{ProSe}{Proximity Services}
  \acro{PS}{Packet Scheduling}
  \acro{PSO}{Particle Swarm Optimization}
  \acro{PZF}{Projected Zero-Forcing}
  \acro{QAM}{Quadrature Amplitude Modulation}
  \acro{QoS}{Quality of Service}
  \acro{QPSK}{Quadri-Phase Shift Keying}
  \acro{RAISES}{Reallocation-based Assignment for Improved Spectral Efficiency and Satisfaction}
  \acro{RAN}{Radio Access Network}
  \acro{RA}{Resource Allocation}
  \acro{RAT}{Radio Access Technology}
  \acro{RATE}{Rate-based}
  \acro{RB}{resource block}
  \acro{RBG}{Resource Block Group}
  \acro{REF}{Reference Grouping}
  \acro{RLC}{Radio Link Control}
  \acro{RM}{Rate Maximization}
  \acro{RNC}{Radio Network Controller}
  \acro{RND}{Random Grouping}
  \acro{RRA}{Radio Resource Allocation}
  \acro{RRM}{Radio Resource Management}
  \acro{RSCP}{Received Signal Code Power}
  \acro{RSRP}{Reference Signal Receive Power}
  \acro{RSRQ}{Reference Signal Receive Quality}
  \acro{RR}{Round Robin}
  \acro{RRC}{Radio Resource Control}
  \acro{RSSI}{Received Signal Strength Indicator}
  \acro{RT}{Real Time}
  \acro{RU}{Resource Unit}
  \acro{RUNE}{RUdimentary Network Emulator}
  \acro{RV}{Random Variable}
  \acro{RZF}{regularized zero forcing}
  \acro{SAC}{Session Admission Control}
  \acro{SCM}{Spatial Channel Model}
  \acro{SC-FDMA}{Single Carrier - Frequency Division Multiple Access}
  \acro{SD}{Soft Dropping}
  \acro{S-D}{Source-Destination}
  \acro{SDPC}{Soft Dropping Power Control}
  \acro{SDMA}{Space-Division Multiple Access}
  \acro{SER}{Symbol Error Rate}
  \acro{SES}{Simple Exponential Smoothing}
  \acro{S-GW}{Serving Gateway}
  \acro{SINR}{signal-to-interference-plus-noise ratio}
  \acro{SI}{Satisfaction Indicator}
  \acro{SIP}{Session Initiation Protocol}
  \acro{SISO}{single input single output}
  \acro{SIMO}{Single Input Multiple Output}
  \acro{SIR}{signal-to-interference ratio}
  \acro{SLNR}{Signal-to-Leakage-plus-Noise Ratio}
  \acro{SMA}{Simple Moving Average}
  \acro{SNR}{signal-to-noise ratio}
  \acro{SORA}{Satisfaction Oriented Resource Allocation}
  \acro{SORA-NRT}{Satisfaction-Oriented Resource Allocation for Non-Real Time Services}
  \acro{SORA-RT}{Satisfaction-Oriented Resource Allocation for Real Time Services}
  \acro{SPF}{Single-Carrier Proportional Fair}
  \acro{SRA}{Sequential Removal Algorithm}
  \acro{SRS}{Sounding Reference Signal}
  \acro{SU-MIMO}{Single-User Multiple Input Multiple Output}
  \acro{SU}{Single-User}
  \acro{SVD}{Singular Value Decomposition}
  \acro{TCP}{Transmission Control Protocol}
  \acro{TDD}{time division duplexing}
  \acro{TDMA}{Time Division Multiple Access}
  \acro{TETRA}{Terrestrial Trunked Radio}
  \acro{TP}{Transmit Power}
  \acro{TPC}{Transmit Power Control}
  \acro{TTI}{Transmission Time Interval}
  \acro{TTR}{Time-To-Rendezvous}
  \acro{TSM}{Throughput-based Satisfaction Maximization}
  \acro{TU}{Typical Urban}
  \acro{UE}{user equipment}
  \acro{UEPS}{Urgency and Efficiency-based Packet Scheduling}
  \acro{UL}{uplink}
  \acro{ULA}{uniform linear array}
  \acro{UMTS}{Universal Mobile Telecommunications System}
  \acro{URI}{Uniform Resource Identifier}
  \acro{URM}{Unconstrained Rate Maximization}
  \acro{UT}{user terminal}
  \acro{VR}{Virtual Resource}
  \acro{VoIP}{Voice over IP}
  \acro{WAN}{Wireless Access Network}
  \acro{WCDMA}{Wideband Code Division Multiple Access}
  \acro{WF}{Water-filling}
  \acro{WiMAX}{Worldwide Interoperability for Microwave Access}
  \acro{WINNER}{Wireless World Initiative New Radio}
  \acro{WLAN}{Wireless Local Area Network}
  \acro{WMPF}{Weighted Multicarrier Proportional Fair}
  \acro{WPF}{Weighted Proportional Fair}
  \acro{WSN}{Wireless Sensor Network}
  \acro{WWW}{World Wide Web}
  \acro{XIXO}{(Single or Multiple) Input (Single or Multiple) Output}
  \acro{ZF}{zero-forcing}
  \acro{ZMCSCG}{Zero Mean Circularly Symmetric Complex Gaussian}
\end{acronym}
%\end{singlespace}



==> MetaFiles/myref.tex <==
% This file was created with JabRef 2.10.
% Encoding: Cp1252


@article{li2018learning,
  title={Learning {IoT} in edge: Deep learning for the Internet of Things with edge computing},
  author={Li, He and Ota, Kaoru and Dong, Mianxiong},
  journal={IEEE Network},
  volume={32},
  number={1},
  pages={96--101},
  year={2018},
  publisher={IEEE}
}

@article{koh2007interior,
  title={An interior-point method for large-scale l1-regularized logistic regression},
  author={Koh, Kwangmoo and Kim, Seung-Jean and Boyd, Stephen},
  journal={Journal of Machine Learning Research},
  volume={8},
  number={Jul},
  pages={1519--1555},
  year={2007}
}

@book{bertsekas1989parallel,
  title={Parallel and distributed computation: numerical methods},
  author={Bertsekas, Dimitri P and Tsitsiklis, John N},
  volume={23},
  year={1989},
  publisher={Prentice hall Englewood Cliffs, NJ}
}


@book{boydcnvx,
author = {Boyd, Stephen and Vandenberghe, Lieven},
title = {Convex Optimization},
year = {2004},
isbn = {0521833787},
publisher = {Cambridge University Press},
address = {USA}
}


@article{IEEE802.11Standard,
author={},
journal={IEEE Std 802.11-2016 (Revision of IEEE Std 802.11-2012)},
title={{{IEEE} Standard for Information technology—Telecommunications and information exchange between systems Local and metropolitan area networks—Specific requirements - Part 11: Wireless {LAN} Medium Access Control ({MAC}) and Physical Layer ({PHY}) Specifications}},
year={2016},
volume={},
number={},
pages={1-3534},
ISSN={null},
month={Dec},}

@article{jordan2015machine,
  title={Machine learning: {T}rends, perspectives, and prospects},
  author={Jordan, Michael I and Mitchell, Tom M},
  journal={Science},
  volume={349},
  number={6245},
  pages={255--260},
  year={2015},
  publisher={American Association for the Advancement of Science}
}

@article{zhang2019deep,
  title={Deep learning in mobile and wireless networking: A survey},
  author={Zhang, Chaoyun and Patras, Paul and Haddadi, Hamed},
  journal={IEEE Communications Surveys \& Tutorials},
  year={2019},
  publisher={IEEE}
}

@article{yu2018parallel,
  title={Parallel restarted {SGD} for non-convex optimization with faster convergence and less communication},
  author={Yu, Hao and Yang, Sen and Zhu, Shenghuo},
  journal={arXiv preprint arXiv:1807.06629},
  year={2018}
}


@inproceedings{chen2013combinatorial,
  title={Combinatorial multi-armed bandit: {G}eneral framework and applications},
  author={Chen, Wei and Wang, Yajun and Yuan, Yang},
  booktitle={International Conference on Machine Learning},
  pages={151--159},
  year={2013}
}

@book{nesterov2013introductory,
  title={Introductory lectures on convex optimization: A basic course},
  author={Nesterov, Yurii},
  volume={87},
  year={2013},
  publisher={Springer Science \& Business Media}
}

@article{duchi2015optimal,
  title={Optimal rates for zero-order convex optimization: {T}he power of two function evaluations},
  author={Duchi, John C and Jordan, Michael I and Wainwright, Martin J and Wibisono, Andre},
  journal={IEEE Transactions on Information Theory},
  volume={61},
  number={5},
  pages={2788--2806},
  year={2015},
  publisher={IEEE}
}

@article{laufer2018hybrid,
  title={A Hybrid Approach for Speaker Tracking Based on {TDOA} and Data-Driven Models},
  author={Laufer-Goldshtein, Bracha and Talmon, Ronen and Gannot, Sharon},
  journal={IEEE/ACM Trans. Audio, Speech, Language Process.},
  volume={26},
  number={4},
  month={Apr.},
  pages={725--735},
  year={2018},
}

@Article{adhikary2013joint,
  Title                    = {Joint spatial division and multiplexing--the large-scale array regime},
  Author                   = {Adhikary, Ansuman and Nam, Junyoung and Ahn, J and Caire, Giuseppe},
  Journal                  = {{IEEE} Trans. Inform. Theory},
  Year                     = {2013},
  Month                    = {Feb.},
  Number                   = {10},
  Pages                    = {6441--6463},
  Volume                   = {59},

  File                     = {#F#}
}

@Article{Adhikary2014JSmmW,
  Title                    = {Joint Spatial Division and Multiplexing for {mm-Wave} Channels},
  Author                   = {A. Adhikary and E. Safadi and M. Samimi and R. Wang and G. Caire and T.S. Rappaport and A.F. Molisch},
  Journal                  = {{IEEE} J. Select. Areas Commun.},
  Year                     = {2014},

  Month                    = {Jun.},
  Number                   = {6},
  Pages                    = {1239--1255},
  Volume                   = {32},
  File                     = {#F#}
}

@article{hou2008spectrum,
  title={Spectrum sharing for multi-hop networking with cognitive radios},
  author={Hou, Y Thomas and Shi, Yi and Sherali, Hanif D},
  journal={{IEEE} J. Select. Areas Commun.},
  volume={26},
  number={1},
  year={2008},
  month={Jan}
}

@Article{ajtai1980note,
  Title                    = {A note on {Ramsey} numbers},
  Author                   = {Ajtai, Mikl{\'o}s and Koml{\'o}s, J{\'a}nos and Szemer{\'e}di, Endre},
  Journal                  = {Journal of Combinatorial Theory, Series A},
  Year                     = {1980},
  Number                   = {3},
  Pages                    = {354--360},
  Volume                   = {29}
}

@Article{Akdeniz2014MillimeterWave,
  Title                    = {Millimeter Wave Channel Modeling and Cellular Capacity Evaluation},
  Author                   = {Akdeniz, M.R. and Yuanpeng Liu and Samimi, M.K. and Shu Sun and Rangan, S. and Rappaport, T.S. and Erkip, E.},
  Journal                  = {{IEEE} J. Sel. Areas Commun.},
  Year                     = {2014},

  Month                    = {Jun.},
  Number                   = {6},
  Pages                    = {1164--1179},
  Volume                   = {32}
}

@Article{alejos2008measurement,
  Title                    = {Measurement and analysis of propagation mechanisms at 40 {GHz}: {V}iability of site shielding forced by obstacles},
  Author                   = {Alejos, Ana V{\'a}zquez and S{\'a}nchez, Manuel Garc{\'\i}a and Cui{\~n}as, I{\~n}igo},
  Journal                  = {{IEEE} Trans. Veh. Technol.},
  Year                     = {2008},

  Month                    = {Nov.},
  Number                   = {6},
  Pages                    = {3369--3380},
  Volume                   = {57}
}

@Article{Alkhateeb2014MIMO,
  Title                    = {{MIMO} Precoding and Combining Solutions for Millimeter-Wave Systems},
  Author                   = {A. Alkhateeb and J. Mo and N. González-Prelcic and R. Heath},
  Journal                  = {{IEEE} Commun. Mag.},
  Year                     = {2014},

  Month                    = {Dec.},
  Number                   = {12},
  Pages                    = {122--130},
  Volume                   = {52},

  File                     = {#F#}
}

@Book{allen1994building,
  Title                    = {Building Penetration Loss Measurements at 900 {MHz}, 11.4 {GHz}, and 28.8 {MHz}},
  Author                   = {Allen, Kenneth C and DeMinco, N and Hoffman, JR and Lo, Y and Papazian, PB},
  Publisher                = {{US} Department of Commerce, National Telecommunications and Information Administration Rep. 94-306},
  Year                     = {1994}
}

@Article{alouini1999area,
  Title                    = {Area spectral efficiency of cellular mobile radio systems},
  Author                   = {Alouini, M-S and Goldsmith, Andrea J},
  Journal                  = {{IEEE} Trans. Veh. Technol.},
  Year                     = {1999},

  Month                    = {Jul.},
  Number                   = {4},
  Pages                    = {1047--1066},
  Volume                   = {48}
}

@InProceedings{an2008directional,
  Title                    = {Directional {MAC} protocol for millimeter wave based wireless personal area networks},
  Author                   = {An, Xueli and Hekmat, Ramin},
  Booktitle                = {Proc. {IEEE} Vehicular Technology Conference (VTC Spring)},
  Year                     = {2008},
  Pages                    = {1636--1640}
}

@Article{andrews2011tractable,
  Title                    = {A tractable approach to coverage and rate in cellular networks},
  Author                   = {G.J. Andrews and F. Baccelli and R.K. Ganti},
  Journal                  = {{IEEE} Trans. Commun.},
  Year                     = {2011},

  Month                    = {Nov.},
  Number                   = {11},
  Pages                    = {3122--3134},
  Volume                   = {59}
}

@Article{Andrews2014What,
  Title                    = {What will {5G} be?},
  Author                   = {Andrews, Jeffrey G and Buzzi, Stefano and Choi, Wan and Hanly, Stephen and Lozano, Angel and Soong, Anthony CK and Zhang, Jianzhong Charlie},
  Journal                  = {{IEEE} J. Select. Areas Commun.},
  Year                     = {2014},

  Month                    = {Jun.},
  Number                   = {6},
  Pages                    = {1065--1082},
  Volume                   = {32},

  File                     = {#F#}
}

@Article{andrews2014overview,
  Title                    = {An overview of load balancing in {HetNets}: {O}ld myths and open problems},
  Author                   = {Andrews, Jeffrey G and Singh, Sarabjot and Ye, Qiaoyang and Lin, Xingqin and Dhillon, Harpreet S},
  Journal                  = {{IEEE} Wireless Commun.},
  Year                     = {2014},

  Month                    = {Apr.},
  Number                   = {2},
  Pages                    = {18--25},
  Volume                   = {21}
}

@Article{astely2013lte,
  Title                    = {{LTE} release 12 and beyond},
  Author                   = {Astely, David and Dahlman, Erik and Fodor, Gabor and Parkvall, Stefan and Sachs, Joachim},
  Journal                  = {{IEEE} Commun. Mag.},
  Year                     = {2013},

  Month                    = {Jul.},
  Number                   = {7},
  Pages                    = {154--160},
  Volume                   = {51}
}

@Article{Athanasiou2014Auction,
  Title                    = {Auction-based Resource Allocation in Millimeter-Wave Wireless Access Networks},
  Author                   = {G. Athanasiou and C. Weeraddana and C. Fischione},
  Journal                  = {{IEEE} Commun. Lett.},
  Year                     = {2013},

  Month                    = {Nov.},
  Number                   = {11},
  Pages                    = {2108--2111},
  Volume                   = {17},

  File                     = {#F#}
}

@Article{Athanasiou2015,
  Title                    = {Optimizing Client Association in {60 GHz} Wireless Access Networks},
  Author                   = {G. Athanasiou and C. Weeraddana and C. Fischione and L. Tassiulas},
  Journal                  = {{IEEE/ACM} Trans. Netw.},
  Year                     = {2015},

  Month                    = {Jun.},
  Number                   = {3},
  Pages                    = {836--850},
  Volume                   = {23},

  File                     = {#F#}
}

@Article{Athanasiou-etal-2013,
  Title                    = {Optimizing Client Association in {60 GHz} Wireless Access Networks},
  Author                   = {G. Athanasiou and C. Weeraddana and C. Fischione and L. Tassiulas},
  Journal                  = {{IEEE/ACM} Trans. Netw.},
  Year                     = {2015},

  Month                    = {Jun.},
  Number                   = {3},
  Pages                    = {836--850},
  Volume                   = {23},

  File                     = {#F#}
}

@InProceedings{Ayach2012Capacity,
  Title                    = {The capacity optimality of beam steering in large millimeter wave {MIMO} systems},
  Author                   = {O. E. Ayach and R. W. Heath and S. Abu-Surra and S. Rajagopal and Z. Pi},
  Booktitle                = {Proc. IEEE International Workshop on Signal Processing Advances in Wireless Communications},
  Year                     = {2012},
  Pages                    = {100--104}
}

@Book{baccelli2009stochastic,
  Title                    = {Stochastic Geometry and Wireless Networks, Volume II--Applications},
  Author                   = {Baccelli, Fran{\c{c}}ois and Blaszczyszyn, Bartlomiej},
  Publisher                = {NOW publishers},
  Year                     = {2009}
}

@Article{badia2008general,
  Title                    = {A general interference-aware framework for joint routing and link scheduling in wireless mesh networks},
  Author                   = {Badia, Leonardo and Erta, Alessandro and Lenzini, Luciano and Zorzi, Michele},
  Journal                  = {{IEEE} Netw.},
  Year                     = {2008},

  Month                    = {Jan.},
  Number                   = {1},
  Pages                    = {32--38},
  Volume                   = {22}
}

@Article{bai2014coverage,
  Title                    = {Coverage and capacity of millimeter-wave cellular networks},
  Author                   = {T. Bai and A. Alkhateeb and R. Heath},
  Journal                  = {{IEEE} Commun. Mag.},
  Year                     = {2014},

  Month                    = {Sept.},
  Number                   = {9},
  Pages                    = {70--77},
  Volume                   = {52}
}

@Article{TBai2014Coverage,
  Title                    = {Coverage and Rate Analysis for Millimeter Wave Cellular Networks},
  Author                   = {T. Bai and R. Heath},
  Journal                  = {{IEEE} Trans. Wireless Commun.},
  Year                     = {2015},

  Month                    = {Feb.},
  Number                   = {2},
  Pages                    = {1100--1114},
  Volume                   = {14},

  File                     = {#F#}
}

@Article{TBai2014Blockage,
  Title                    = {Analysis of blockage effects on urban cellular networks},
  Author                   = {T. Bai and R. Vaze and R. Heath},
  Journal                  = {{IEEE} Trans. Wireless Commun.},
  Year                     = {2014},

  Month                    = {Sept.},
  Number                   = {9},
  Pages                    = {5070--5083},
  Volume                   = {13},

  File                     = {#F#}
}

@Book{balanis2012antenna,
  Title                    = {Antenna theory: {A}nalysis and design},
  Author                   = {Balanis, Constantine A},
  Publisher                = {John Wiley \& Sons},
  Year                     = {2012}
}

@Article{Baldemair2015Ultra,
  Title                    = {Ultra-Dense Networks in Millimeter-Wave Frequencies},
  Author                   = {R. Baldemair and T. Irnich and K. Balachandran and E. Dahlman and G. Mildh and Y. Selen and S. Parkvall and M. Meyer and A. Osseiran},
  Journal                  = {{IEEE} Commun. Mag.},
  Year                     = {2015},

  Month                    = {Jan.},
  Number                   = {1},
  Pages                    = {202--208},
  Volume                   = {53},

  File                     = {#F#}
}

@Article{Bazan2012Survey,
  Title                    = {A Survey On {MAC} Protocols for Wireless Adhoc Networks with Beamforming Antennas},
  Author                   = {O. Bazan and M. Jaseemuddin},
  Journal                  = {{IEEE} Commun. Surveys Tuts.},
  Year                     = {2012},

  Month                    = {Second Quarter},
  Number                   = {2},
  Pages                    = {1513--1527},
  Volume                   = {14},

  File                     = {#F#}
}

@Book{benvenuto2011principles,
  Title                    = {Principles of communications Networks and Systems},
  Author                   = {Benvenuto, Nevio and Zorzi, Michele},
  Publisher                = {Wiley Online Library},
  Year                     = {2011}
}

@Article{bhattacharyya1946measure,
  Title                    = {On a measure of divergence between two multinomial populations},
  Author                   = {Bhattacharyya, Anil},
  Journal                  = {Sankhy{\=a}: The Indian Journal of Statistics},
  Year                     = {1946},

  Month                    = {Jul.},
  Number                   = {4},
  Pages                    = {401--406},
  Volume                   = {7}
}

@Article{bhushan2014network,
  Title                    = {Network densification: {T}he dominant theme for wireless evolution into {5G}},
  Author                   = {Bhushan, Naga and Li, Junyi and Malladi, Durga and Gilmore, Rob and Brenner, Dean and Damnjanovic, Aleksandar and Sukhavasi, Ravi and Patel, Chirag and Geirhofer, Stefan},
  Journal                  = {{IEEE} Commun. Mag.},
  Year                     = {2014},

  Month                    = {Feb.},
  Number                   = {2},
  Pages                    = {82--89},
  Volume                   = {52}
}

@Article{bianchi2000performance,
  Title                    = {Performance analysis of the {IEEE 802.11} distributed coordination function},
  Author                   = {Bianchi, Giuseppe},
  Journal                  = {{IEEE} J. Sel. Areas Commun.},
  Year                     = {2000},

  Month                    = {Mar.},
  Number                   = {3},
  Pages                    = {535--547},
  Volume                   = {18}
}

@InProceedings{bjorklund2003resource,
  Title                    = {Resource optimization of spatial TDMA in ad hoc radio networks: {A} column generation approach},
  Author                   = {Bjorklund, Patrik and Varbrand, Peter and Yuan, Di},
  Booktitle                = {Proc. {IEEE} International Conference on Computer Communications (INFOCOM)},
  Year                     = {2003},
  Pages                    = {818--824}
}

@Article{boccardi2014Five,
  Title                    = {Five Disruptive Technology Directions for {5G}},
  Author                   = {Boccardi, Federico and Heath, Robert and Lozano, Angel and Marzetta, Thomas L and Popovski, Petar},
  Journal                  = {{IEEE} Commun. Mag.},
  Year                     = {2014},

  Month                    = {Feb.},
  Number                   = {2},
  Pages                    = {74--80},
  Volume                   = {52}
}

@Article{Bogale2015Hybrid,
  Title                    = {Hybrid Analog-Digital Channel Estimation and Beamforming: {T}raining-Throughput Tradeoff},
  Author                   = {Tadilo Endeshaw Bogale and Long Bao Le and Xianbin Wang},
  Journal                  = {{IEEE} Trans. Commun.},
  Year                     = {2015},

  Month                    = {Dec.},
  Number                   = {12},
  Pages                    = {5235--5249},
  Volume                   = {63}
}

@Book{bollobas1998random,
  Title                    = {Random graphs},
  Author                   = {Bollob{\'a}s, B{\'e}la},
  Publisher                = {Springer},
  Year                     = {1998}
}

@Book{bondy1976graph,
  Title                    = {Graph theory with applications},
  Author                   = {Bondy, John Adrian and Murty, Uppaluri Siva Ramachandra},
  Publisher                = {Macmillan London},
  Year                     = {1976},
  Volume                   = {290}
}

@Article{bubeck2012regret,
  Title                    = {Regret analysis of stochastic and nonstochastic multi-armed bandit problems},
  Author                   = {Bubeck, S{\'e}bastien and Cesa-Bianchi, Nicolo and others},
  Journal                  = {Foundations and Trends{\textregistered} in Machine Learning},
  Year                     = {2012},
  Number                   = {1},
  Pages                    = {1--122},
  Volume                   = {5},

  Publisher                = {Now Publishers, Inc.}
}

@Article{cardieri2010modeling,
  Title                    = {Modeling interference in wireless ad hoc networks},
  Author                   = {Cardieri, Paulo},
  Journal                  = {{IEEE} Commun. Surveys Tuts.},
  Year                     = {2010},

  Month                    = {Fourth Quarter},
  Number                   = {4},
  Pages                    = {551--572},
  Volume                   = {12}
}

@Article{celik2010mac,
  Title                    = {{MAC} for networks with multipacket reception capability and spatially distributed nodes},
  Author                   = {Celik, Guner D and Zussman, Gil and Khan, Wajahat F and Modiano, Eytan},
  Journal                  = {{IEEE} Trans. Mobile Comput.},
  Year                     = {2010},

  Month                    = {Aug.},
  Number                   = {2},
  Pages                    = {226--240},
  Volume                   = {9}
}

@Article{chai2014low,
  Title                    = {Low-Overhead Control Channels in Wireless Networks},
  Author                   = {Chai, Eugene and Shin, K},
  Journal                  = {{IEEE} Trans. Mobile Comput.},
  Year                     = {2015},
  Note                     = {to be published}
}

@Article{chandrasekhar2009power,
  Title                    = {Power control in two-tier femtocell networks},
  Author                   = {Chandrasekhar, Vikram and Andrews, Jeffrey G and Muharemovic, Tarik and Shen, Zukang and Gatherer, Alan},
  Journal                  = {{IEEE} Trans. Wireless Commun.},
  Year                     = {2009},

  Month                    = {Aug.},
  Number                   = {8},
  Pages                    = {4316--4328},
  Volume                   = {8}
}

@Article{Cheung2012Throughput,
  Title                    = {Throughput optimization, spectrum allocation, and access control in two-tier femtocell networks},
  Author                   = {W. C. Cheung and T. Quek and M. Kountouris},
  Journal                  = {{IEEE} J. Sel. Areas Commun.},
  Year                     = {2012},

  Month                    = {Apr.},
  Number                   = {3},
  Pages                    = {561--574},
  Volume                   = {30}
}

@Article{choi2007downlink,
  Title                    = {Downlink performance and capacity of distributed antenna systems in a multicell environment},
  Author                   = {Choi, Wan and Andrews, Jeffrey G},
  Journal                  = {Wireless Communications, IEEE Transactions on},
  Year                     = {2007},
  Number                   = {1},
  Pages                    = {69--73},
  Volume                   = {6}
}

@Book{cramer2004random,
  Title                    = {Random variables and probability distributions},
  Author                   = {Cram{\'e}r, Harald},
  Publisher                = {Cambridge University Press},
  Year                     = {2004},
  Volume                   = {36}
}

@Article{dahrouj2010coordinated,
  Title                    = {Coordinated beamforming for the multicell multi-antenna wireless system},
  Author                   = {Dahrouj, Hayssam and Yu, Wei},
  Journal                  = {{IEEE} Trans. Wireless Commun.},
  Year                     = {2010},

  Month                    = {May},
  Number                   = {5},
  Pages                    = {1748--1759},
  Volume                   = {9}
}

@Book{daley2007introduction,
  Title                    = {An introduction to the theory of point processes},
  Author                   = {Daley, Daryl J and Vere-Jones, David},
  Publisher                = {Springer Science \& Business Media},
  Year                     = {2007},
  Volume                   = {2}
}

@InProceedings{dani2008price,
  Title                    = {The price of bandit information for online optimization},
  Author                   = {Dani, Varsha and Kakade, Sham M and Hayes, Thomas P},
  Booktitle                = {Advances in Neural Information Processing Systems},
  Year                     = {2008},
  Pages                    = {345--352}
}

@Book{david1970order,
  Title                    = {Order statistics},
  Author                   = {David, Herbert Aron and Nagaraja, Haikady Navada},
  Publisher                = {Wiley Online Library},
  Year                     = {2003},
  Note                     = {Third Edition}
}

@Article{David1965Exact,
  Title                    = {Exact Distribution of the Sum of Independent Identically Distributed Discrete Random Variables},
  Author                   = {David, H. A. and Norman, J. E.},
  Journal                  = {Journal of the American Statistical Association},
  Year                     = {1965},

  Month                    = {Sept.},
  Number                   = {311},
  Pages                    = {837--842},
  Volume                   = {60}
}

@Article{dehos2014millimeter,
  Title                    = {Millimeter-wave access and backhauling: {T}he solution to the exponential data traffic increase in {5G} mobile communications systems?},
  Author                   = {C. Dehos and J. Gonzalez and A. Domenico and D. Ktenas and L. Dussopt},
  Journal                  = {{IEEE} Commun. Mag.},
  Year                     = {2014},

  Month                    = {Sept.},
  Number                   = {9},
  Pages                    = {88--95},
  Volume                   = {52}
}

@Article{demestichas20135g,
  Title                    = {{5G} on the horizon: {Key} challenges for the radio-access network},
  Author                   = {Demestichas, Panagiotis and Georgakopoulos, Andreas and Karvounas, Dimitrios and Tsagkaris, Kostas and Stavroulaki, Vera and Lu, Jianmin and Xiong, Chunshan and Yao, Jing},
  Journal                  = {{IEEE} Veh. Technol. Mag.},
  Year                     = {2013},

  Month                    = {Sept.},
  Number                   = {3},
  Pages                    = {47--53},
  Volume                   = {8}
}

@Article{dhillon2012modeling,
  Title                    = {Modeling and analysis of K-tier downlink heterogeneous cellular networks},
  Author                   = {Dhillon, Harpreet S and Ganti, Radha Krishna and Baccelli, Fran{\c{c}}ois and Andrews, Jeffrey G},
  Journal                  = {{IEEE} J. Sel. Areas Commun.},
  Year                     = {2012},

  Month                    = {Apr.},
  Number                   = {3},
  Pages                    = {550--560},
  Volume                   = {30}
}

@Article{di2014stochastic,
  Title                    = {Stochastic Geometry Modeling and Analysis of Multi-Tier Millimeter Wave Cellular Networks},
  Author                   = {Di Renzo, Marco},
  Journal                  = {{IEEE} Trans. Wireless Commun.},
  Year                     = {2015},

  Month                    = {Sept.},
  Number                   = {9},
  Pages                    = {5038--5057},
  Volume                   = {14}
}

@InProceedings{ECMA387,
  Title                    = {High rate 60 {GHz} {PHY}, {MAC} and {HDMI} {PAL}},
  Author                   = {{ECMA-TC48, ECMA standard 387}},
  Year                     = {2008},
  Month                    = {Dec.}
}

@Article{el2014spatially,
  Title                    = {Spatially sparse precoding in millimeter wave {MIMO} systems},
  Author                   = {El Ayach, Omar and Rajagopal, Sridhar and Abu-Surra, Shadi and Pi, Zhouyue and Heath, R},
  Journal                  = {{IEEE} Trans. Wireless Commun.},
  Year                     = {2014},

  Month                    = {Mar.},
  Number                   = {3},
  Pages                    = {1499--1513},
  Volume                   = {13},

  File                     = {#F#}
}

@Article{el2006optimal,
  Title                    = {Optimal throughput-delay scaling in wireless networks--part {I}: {T}he fluid model},
  Author                   = {El Gamal, Abbas and Mammen, James and Prabhakar, Balaji and Shah, Devavrat},
  Journal                  = {{IEEE} Trans. Inform. Theory},
  Year                     = {2006},

  Month                    = {Jun.},
  Number                   = {6},
  Pages                    = {2568--2592},
  Volume                   = {52}
}

@Article{elshaer2016downlink,
  Title                    = {Downlink and Uplink Cell Association with Traditional Macrocells and Millimeter Wave Small Cells},
  Author                   = {Elshaer, Hisham and Kulkarni, Mandar and Boccardi, Federico and Andrews, Jeffrey and Dohler, Mischa},
  Journal                  = {{IEEE} Trans. Wireless Commun.},
  Year                     = {2016},
  Note                     = {To appear}
}

@Article{ephremides1982analysis,
  Title                    = {Analysis of a hybrid access scheme for buffered users-probabilistic time division},
  Author                   = {Ephremides, Anthony and Mowafi, Osama A.},
  Journal                  = {{IEEE} Trans. Software Eng.},
  Year                     = {1982},

  Month                    = {Jan.},
  Number                   = {1},
  Pages                    = {52--61}
}

@Article{FCC3,
  Title                    = {{81-FR-1801}},
  Author                   = {{Federal Communications Commission}},
  Year                     = {2016},

  Month                    = {Jan.},

  Url                      = {https://www.gpo.gov/fdsys/pkg/FR-2016-01-13/pdf/2015-31852.pdf}
}

@Article{FCC2,
  Title                    = {{FCC-177}},
  Author                   = {{Federal Communications Commission}},
  Year                     = {2015},

  Month                    = {Jan.},

  Url                      = {http://apps.fcc.gov/ecfs/proceeding/view?name=14-177}
}

@Article{FCC1,
  Title                    = {{FCC-154}},
  Author                   = {{Federal Communications Commission}},
  Year                     = {2014},

  Month                    = {Oct.},

  Url                      = {http://apps.fcc.gov/edocs public/attachmatch/FCC-14-154A1.pdf}
}

@InProceedings{Feng2014InterNetwork,
  Title                    = {Inter-network spatial sharing with interference mitigation based on {IEEE} 802.11ad {WLAN} system},
  Author                   = {W. Feng and Y. Li and D. Jin and L. Zeng},
  Booktitle                = {Proc. {IEEE} Global Communications Conference (GLOBECOM) Workshop},
  Year                     = {2014},
  Month                    = {Dec.},
  Pages                    = {725--758}
}

@Article{Fischione2013Dynamic,
  Title                    = {Dynamic Optimization of Generalized Least Squares Handover Algorithms},
  Author                   = {C. Fischione and G. Athanasiou and F. Santucci},
  Journal                  = {{IEEE} Trans. Wireless Commun.},
  Year                     = {2014},

  Month                    = {Mar.},
  Number                   = {3},
  Pages                    = {1235--1248},
  Volume                   = {13},

  File                     = {#F#}
}

@InProceedings{Fodor2014Performance,
  Title                    = {Performance Analysis of Block and Comb Type Channel Estimation for Massive {MIMO} Systems},
  Author                   = {G. Fodor and P. {Di Marco} and M. Telek},
  Booktitle                = {Proc. {IEEE} International Conference on 5G for Ubiquitous Connectivity (5GU)},
  Year                     = {2014},
  Pages                    = {62--69}
}

@Article{fodor2012design,
  Title                    = {Design aspects of network assisted device-to-device communications},
  Author                   = {Fodor, G{\'a}bor and Dahlman, Erik and Mildh, Gunnar and Parkvall, Stefan and Reider, Norbert and Mikl{\'o}s, Gy{\"o}rgy and Tur{\'a}nyi, Zolt{\'a}n},
  Journal                  = {{IEEE} Commun. Mag.},
  Year                     = {2012},

  Month                    = {Mar.},
  Number                   = {3},
  Pages                    = {170--177},
  Volume                   = {50}
}

@InProceedings{fodor2014pilot,
  Title                    = {On the pilot-data power trade off in single input multiple output systems},
  Author                   = {Fodor, G{\'a}bor and Telek, Mikl{\'o}s},
  Booktitle                = {Proc. 20th European Wireless (EW) Conference},
  Year                     = {2014},
  Pages                    = {1--8}
}

@InProceedings{gamal2004throughput,
  Title                    = {Throughput-delay trade-off in wireless networks},
  Author                   = {Gamal, A El and Mammen, James and Prabhakar, Bharat and Shah, Devavrat},
  Booktitle                = {Proc. {IEEE} International Conference on Computer Communications (INFOCOM)},
  Year                     = {2004},
  Pages                    = {464--475}
}

@InProceedings{ganti2009bounds,
  Title                    = {Bounds on the information propagation delay in interference-limited aloha networks},
  Author                   = {Ganti, Radha Krishna and Haenggi, Martin},
  Booktitle                = {Proc. Modeling and Optimization in Mobile, Ad Hoc, and Wireless Networks (WiOPT)},
  Year                     = {2009},
  Pages                    = {1--7}
}

@InProceedings{ganti2007dynamic,
  Title                    = {Dynamic connectivity and packet propagation delay in {ALOHA} wireless networks},
  Author                   = {Ganti, Radha Krishna and Haenggi, Martin},
  Booktitle                = {Proc. {IEEE} Asilomar Conference on Signals, Systems and Computers (ACSSC)},
  Year                     = {2007},
  Pages                    = {143--147}
}

@Article{garetto2008modeling,
  Title                    = {Modeling per-flow throughput and capturing starvation in {CSMA} multi-hop wireless networks},
  Author                   = {Garetto, Michele and Salonidis, Theodoros and Knightly, Edward W},
  Journal                  = {{IEEE/ACM} Trans. Netw.},
  Year                     = {2008},

  Month                    = {Aug.},
  Number                   = {4},
  Pages                    = {864--877},
  Volume                   = {16}
}

@Article{garivier2016explore,
  Title                    = {Explore first, exploit next: The true shape of regret in bandit problems},
  Author                   = {Garivier, Aur{\'e}lien and M{\'e}nard, Pierre and Stoltz, Gilles},
  Journal                  = {arXiv preprint arXiv:1602.07182},
  Year                     = {2016}
}

@Article{Shokri2018Interference,
  Title                    = {Interference model similarity index and its applications to millimeter-wave networks},
  Author                   = {H. S. Ghadikolaei and C. Fischione and E. Modinao},
  Journal                  = {{IEEE} Trans. Wireless Commun.},
  Year                     = {2018},

  Month                    = {Jan.},
  Number                   = {1},
  Pages                    = {71--85},
  Volume                   = {17}
}

@Article{Ghauch_SED_16,
  Title                    = {Subspace Estimation and Decomposition for Large Millimeter-Wave MIMO Systems},
  Author                   = {H. Ghauch and T. Kim and M. Bengtsson and M. Skoglund},
  Journal                  = {IEEE Journal of Selected Topics in Signal Processing},
  Year                     = {2016},

  Month                    = {Apr.},
  Number                   = {3},
  Pages                    = {528-542},
  Volume                   = {10},

  Doi                      = {10.1109/JSTSP.2016.2538178},
  ISSN                     = {1932-4553}
}

@Article{goldsmith2003capacity,
  Title                    = {Capacity limits of {MIMO} channels},
  Author                   = {Goldsmith, Andrea and Jafar, Syed Ali and Jindal, Nihar and Vishwanath, Sriram},
  Journal                  = {{IEEE} J. Sel. Areas Commun.},
  Year                     = {2003},

  Month                    = {Jun.},
  Number                   = {5},
  Pages                    = {684--702},
  Volume                   = {21}
}

@Article{goldsmith1997capacity,
  Title                    = {Capacity of fading channels with channel side information},
  Author                   = {Goldsmith, Andrea J and Varaiya, Pravin P},
  Journal                  = {{IEEE} Trans. Inf. Theory},
  Year                     = {1997},

  Month                    = {Nov.},
  Number                   = {6},
  Pages                    = {1986--1992},
  Volume                   = {43}
}

@InProceedings{gronkvist2001comparison,
  Title                    = {Comparison between graph-based and interference-based STDMA scheduling},
  Author                   = {Gr{\"o}nkvist, Jimmi and Hansson, Anders},
  Booktitle                = {Proc. {ACM} international symposium on Mobile ad hoc networking \& computing (MobiHoc)},
  Year                     = {2001},
  Pages                    = {255--258}
}

@InProceedings{guo2014uplink,
  Title                    = {Uplink Power Control with {MMSE} Receiver in Multi-Cell {MU}-Massive-{MIMO} Systems},
  Author                   = {K. Guo and Y. Guo and G. Fodor and G. Ascheid},
  Booktitle                = {Proc. {IEEE} International Conference on Communications (ICC)},
  Year                     = {2014},
  Pages                    = {5184--5190}
}

@Article{Gupta2016Sharing,
  Title                    = {On the feasibility of sharing spectrum licenses in mmWave cellular systems},
  Author                   = {A. K. Gupta and J. G. Andrews and R. W. Heath},
  Journal                  = {arXiv:1512.01290},
  Year                     = {2016}
}

@Article{gupta2000capacity,
  Title                    = {The capacity of wireless networks},
  Author                   = {Gupta, Piyush and Kumar, Panganmala R},
  Journal                  = {{IEEE} Trans. Inform. Theory},
  Year                     = {2000},

  Month                    = {Mar.},
  Number                   = {2},
  Pages                    = {388--404},
  Volume                   = {46}
}

@Book{Haenggi2013Stochastic,
  Title                    = {Stochastic Geometry for Wireless Networks},
  Author                   = {Martin Haenggi},
  Publisher                = {Cambridge University Press},
  Year                     = {2013}
}

@Article{Haenggi2005OnDistance,
  Title                    = {On distances in uniformly random networks},
  Author                   = {Haenggi, Martin},
  Journal                  = {{IEEE} Trans. Inf. Theory},
  Year                     = {2005},

  Month                    = {Oct.},
  Number                   = {10},
  Pages                    = {3584--3586},
  Volume                   = {51}
}

@Article{haenggi2009stochastic,
  Title                    = {Stochastic geometry and random graphs for the analysis and design of wireless networks},
  Author                   = {Haenggi, Martin and Andrews, Jeffrey G and Baccelli, Fran{\c{c}}ois and Dousse, Olivier and Franceschetti, Massimo},
  Journal                  = {{IEEE} J. Sel. Areas Commun.},
  Year                     = {2009},

  Month                    = {Sept.},
  Number                   = {7},
  Pages                    = {1029--1046},
  Volume                   = {27}
}

@Article{haider2014cellular,
  Title                    = {Cellular architecture and key technologies for {5G} wireless communication networks},
  Author                   = {Haider, Fourat and Gao, Xiqi and You, Xiao-Hu and Yang, Yang and Yuan, Dongfeng and Aggoune, Hadi M and Haas, Harald},
  Journal                  = {{IEEE} Commun. Mag.},
  Year                     = {2014},

  Month                    = {Feb.},
  Pages                    = {123--130}
}

@article{de2018high,
  title={High-accuracy low-precision training},
  author={De Sa, Christopher and Leszczynski, Megan and Zhang, Jian and Marzoev, Alana and Aberger, Christopher R and Olukotun, Kunle and R{\'e}, Christopher},
  journal={arXiv preprint arXiv:1803.03383},
  year={2018}
}

@inproceedings{wen2017terngrad,
  title={Terngrad: Ternary gradients to reduce communication in distributed deep learning},
  author={Wen, Wei and Xu, Cong and Yan, Feng and Wu, Chunpeng and Wang, Yandan and Chen, Yiran and Li, Hai},
  booktitle={Advances in Neural Information Processing Systems},
  pages={1509--1519},
  year={2017}
}


@InProceedings{bernstein2018signsgd,
  title = 	 {sign{SGD}: Compressed Optimisation for Non-Convex Problems},
  author = 	 {Bernstein, Jeremy and Wang, Yu-Xiang and Azizzadenesheli, Kamyar and Anandkumar, Animashree},
  booktitle = 	 {Proceedings of the 35th International Conference on Machine Learning},
  pages = 	 {560--569},
  year = 	 {2018},
}

@inproceedings{alistarh2017qsgd,
  title={{QSGD}: Communication-efficient SGD via gradient quantization and encoding},
  author={Alistarh, Dan and Grubic, Demjan and Li, Jerry and Tomioka, Ryota and Vojnovic, Milan},
  booktitle={Advances in Neural Information Processing Systems},
  pages={1709--1720},
  year={2017}
}


@article{magnusson2017convergence,
  title={Convergence of limited communications gradient methods},
  author={Magn{\'u}sson, Sindri and Enyioha, Chinwendu and Li, Na and Fischione, Carlo and Tarokh, Vahid},
  journal={IEEE Transactions on Automatic Control},
  volume = {63},
  number = {5},
  pages = {1351--1371},
  month={May},
  year = {2017},
}

@misc{kairouz2019advances,
    title={Advances and Open Problems in Federated Learning},
    author={Peter Kairouz and others},
    year={2019},
    eprint={1912.04977},
    archivePrefix={arXiv},
    primaryClass={cs.LG}
}

@inproceedings{Defazio2014SAGA,
 author = {Defazio, Aaron and Bach, Francis and Lacoste-Julien, Simon},
 booktitle = {Advances in Neural Information Processing Systems},
 editor = {Z. Ghahramani and M. Welling and C. Cortes and N. Lawrence and K. Q. Weinberger},
 pages = {},
 publisher = {Curran Associates, Inc.},
 title = {SAGA: A Fast Incremental Gradient Method With Support for Non-Strongly Convex Composite Objectives},
 volume = {27},
 year = {2014}
}



@InProceedings{shokri-21-LENA,
  title = 	 {{LENA}: Communication-Efficient Distributed Learning with Self-Triggered Gradient Uploads },
  author =       {S. Ghadikolaei, Hossein and Stich, Sebastian and Jaggi, Martin},
  booktitle = 	 {Proceedings of The 24th International Conference on Artificial Intelligence and Statistics},
  pages = 	 {3943--3951},
  year = 	 {2021},
  volume = 	 {130},
  series = 	 {Proceedings of Machine Learning Research},
  month = 	 {13--15 Apr},
  publisher =    {PMLR},}
}

@inproceedings{mahmoudi2020cost,
  title={Cost-efficient Distributed Optimization in Machine Learning Over Wireless Networks},
  author={Afsaneh Mahmoudi and Hossein S. Ghadikolaei and Carlo Fischione},
  Booktitle = {{IEEE} International Conference on Communications (ICC)},
  year={2020},
}

@inproceedings{mahmoudi20spawc,
  title={Machine Learning over Networks: Co-design of Distributed Optimization and Communications},
  author={Afsaneh Mahmoudi and Hossein S. Ghadikolaei and Carlo Fischione},
  Booktitle = {{IEEE} International Workshop on Signal Processing Advances in Wireless Communications (SPAWC)},
  year={2020},
}
@article{jordan2018communication,
  title={Communication-efficient distributed statistical inference},
  author={Jordan, Michael I and Lee, Jason D and Yang, Yun},
  journal={Journal of the American Statistical Association},
  year={2018},
  publisher={Taylor \& Francis}
}

@inproceedings{johnson2013accelerating,
  title={Accelerating stochastic gradient descent using predictive variance reduction},
  author={Johnson, Rie and Zhang, Tong},
  booktitle={Advances in neural information processing systems},
  pages={315--323},
  year={2013}
}

@article{konevcny2016federated,
  title={Federated learning: {S}trategies for improving communication efficiency},
  author={Kone{\v{c}}n{\`y}, Jakub and McMahan, H Brendan and Yu, Felix X and Richt{\'a}rik, Peter and Suresh, Ananda Theertha and Bacon, Dave},
  journal={arXiv preprint arXiv:1610.05492},
  year={2016}
}

@Article{Hirokawa2000Sidelobe,
  Title                    = {Sidelobe suppression in {76-GHz} post-wall waveguide-fed parallel-plate slot arrays},
  Author                   = {Hirokawa, J. and Ando, M.},
  Journal                  = {{IEEE} Trans. Antennas Propag.},
  Year                     = {2000},

  Month                    = {Nov},
  Number                   = {11},
  Pages                    = {1727-1732},
  Volume                   = {48},

  ISSN                     = {0018-926X}
}

@Article{hsin2006randomly,
  Title                    = {Randomly duty-cycled wireless sensor networks: dynamics of coverage},
  Author                   = {Hsin, Chih-fan and Liu, Mingyan},
  Journal                  = {{IEEE} Trans. Wireless Commun.},
  Year                     = {2006},

  Month                    = {Nov.},
  Number                   = {11},
  Pages                    = {3182--3192},
  Volume                   = {5}
}

@Article{hui2005unified,
  Title                    = {A unified model for the performance analysis of {IEEE} 802.11e {EDCA}},
  Author                   = {Hui, Jie and Devetsikiotis, Michael},
  Journal                  = {{IEEE} Trans. Commun.},
  Year                     = {2005},

  Month                    = {Sept.},
  Number                   = {9},
  Pages                    = {1498--1510},
  Volume                   = {53}
}

@Article{hujtera1993number,
  Title                    = {The number of maximal independent sets in triangle-free graphs},
  Author                   = {Hujtera, Mih{\'a}ly and Tuza, Zsolt},
  Journal                  = {SIAM Journal on Discrete Mathematics},
  Year                     = {1993},
  Number                   = {2},
  Pages                    = {284--288},
  Volume                   = {6}
}

@Article{hunter2008transmission,
  Title                    = {Transmission capacity of ad hoc networks with spatial diversity},
  Author                   = {Hunter, Andrew M and Andrews, Jeffrey G and Weber, Steven},
  Journal                  = {{IEEE} Trans. Wireless Commun.},
  Year                     = {2008},

  Month                    = {Dec.},
  Number                   = {12},
  Pages                    = {5058--5071},
  Volume                   = {7}
}

@InProceedings{Irnich2013SpectrumSharing,
  Title                    = {Spectrum sharing scenarios and resulting technical requirements for {5G} systems},
  Author                   = {T. Irnich and J. Kronander and Y. Selen and G. Li},
  Booktitle                = {Proc. IEEE International Symposium on Personal, Indoor and Mobile Radio Communications (PIMRC)},
  Year                     = {2013},
  Month                    = {Sept.},
  Pages                    = {127--132}
}

@InProceedings{ishii2012novel,
  Title                    = {A novel architecture for {LTE-B}: {C-plane/U-plane} split and {Phantom Cell} concept},
  Author                   = {Ishii, Hiroyuki and Kishiyama, Yoshihisa and Takahashi, Hideaki},
  Booktitle                = {Proc. {IEEE} Globecom Workshops},
  Year                     = {2012},
  Pages                    = {624--630}
}

@Article{iyer2009right,
  Title                    = {What is the right model for wireless channel interference?},
  Author                   = {Iyer, Aravind and Rosenberg, Catherine and Karnik, Aditya},
  Journal                  = {{IEEE} Trans. Wireless Commun.},
  Year                     = {2009},

  Month                    = {May},
  Number                   = {5},
  Pages                    = {2662--2671},
  Volume                   = {8}
}

@Article{jafar2014topological,
  Title                    = {Topological interference management through index coding},
  Author                   = {Jafar, Syed},
  Journal                  = {{IEEE} Trans. Inf. Theory},
  Year                     = {2014},

  Month                    = {Jan.},
  Number                   = {1},
  Pages                    = {529--568},
  Volume                   = {60}
}

@Article{jain2005impact,
  Title                    = {Impact of interference on multi-hop wireless network performance},
  Author                   = {Jain, Kamal and Padhye, Jitendra and Padmanabhan, Venkata N and Qiu, Lili},
  Journal                  = {Wireless Networks},
  Year                     = {2005},
  Number                   = {4},
  Pages                    = {471--487},
  Volume                   = {11}
}

@Article{jain1998quantitative,
  Title                    = {A quantitative measure of fairness and discrimination for resource allocation in shared computer systems},
  Author                   = {R. Jain and D. Chiu and W. Hawe},
  Journal                  = {Digital Equipment Corp., Tech. Rep.},
  Year                     = {1998}
}

@Article{jang2012ieee,
  Title                    = {{IEEE} 802.11 saturation throughput analysis in the presence of hidden terminals},
  Author                   = {Jang, Beakcheol and Sichitiu, Mihail L},
  Journal                  = {{IEEE/ACM} Trans. Netw.},
  Year                     = {2012},

  Month                    = {Apr.},
  Number                   = {2},
  Pages                    = {557--570},
  Volume                   = {20}
}

@Article{Jeong2015Random,
  Title                    = {Random Access in Millimeter-Wave Beamforming Cellular Networks: {I}ssues and Approaches},
  Author                   = {C. Jeong and J. Park and H. Yu},
  Journal                  = {{IEEE} Commun. Mag.},
  Year                     = {2015},

  Month                    = {Jan.},
  Number                   = {1},
  Pages                    = {180--185},
  Volume                   = {53},

  File                     = {#F#}
}

@Article{jiang2010distributed,
  Title                    = {A distributed {CSMA} algorithm for throughput and utility maximization in wireless networks},
  Author                   = {Jiang, Libin and Walrand, Jean},
  Journal                  = {{IEEE/ACM} Trans. Netw.},
  Year                     = {2010},

  Month                    = {Jun.},
  Number                   = {3},
  Pages                    = {960--972},
  Volume                   = {18}
}

@Article{jiang2004asymptotic,
  Title                    = {Asymptotic improvement of the {Gilbert-Varshamov} bound on the size of binary codes},
  Author                   = {Jiang, Tao and Vardy, Alexander},
  Journal                  = {{IEEE} Trans. Inf. Theory},
  Year                     = {2004},

  Month                    = {Aug.},
  Number                   = {8},
  Pages                    = {1655--1664},
  Volume                   = {50}
}

@Article{jo2012heterogeneous,
  Title                    = {Heterogeneous cellular networks with flexible cell association: {A} comprehensive downlink {SINR} analysis},
  Author                   = {Jo, Han-Shin and Sang, Young Jin and Xia, Ping and Andrews, Jeffrey G},
  Journal                  = {{IEEE} Trans. Wireless Commun.},
  Year                     = {2012},

  Month                    = {Oct.},
  Number                   = {10},
  Pages                    = {3484--3495},
  Volume                   = {11}
}

@Book{johnson2005univariate,
  Title                    = {Univariate discrete distributions},
  Author                   = {Johnson, Norman L and Kemp, Adrienne W and Kotz, Samuel},
  Publisher                = {John Wiley \& Sons},
  Year                     = {2005},
  Volume                   = {444}
}

@Article{jones1990size,
  Title                    = {Size and independence in triangle-free graphs with maximum degree three},
  Author                   = {Jones, Kathryn Fraughnaugh},
  Journal                  = {Journal of Graph Theory},
  Year                     = {1990},
  Number                   = {5},
  Pages                    = {525--535},
  Volume                   = {14}
}

@Article{Jorswieck2015Sharing,
  Title                    = {Spectrum sharing improves the network efficiency for cellular operators},
  Author                   = {E. A. Jorswieck and L. Badia and T. Fahldieck and M. Haardt and E. Karipidis and J. Luo and R. Pisz},
  Journal                  = {{IEEE} Commun. Mag.},
  Year                     = {2014},

  Month                    = {Mar.},
  Number                   = {3},
  Pages                    = {129--136},
  Volume                   = {52}
}

@Article{Kailath1967Bhattacharyya,
  Title                    = {The Divergence and {Bhattacharyya} Distance Measures in Signal Selection},
  Author                   = {Kailath, T.},
  Journal                  = {{IEEE} Trans. Commun.},
  Year                     = {1967},

  Month                    = {Feb.},
  Number                   = {1},
  Pages                    = {52--60},
  Volume                   = {15}
}

@Article{Khan2011Network,
  Title                    = {Network sharing in the next mobile network: {TCO} reduction, management flexibility, and operational independence},
  Author                   = {A. Khan and W. Kellerer and K. Kozu and M. Yabusaki},
  Journal                  = {{IEEE} Commun. Mag.},
  Year                     = {2011},

  Month                    = {Oct.},
  Number                   = {10},
  Pages                    = {134--142},
  Volume                   = {49}
}

@Book{Kleinrock1976Queueing,
  Title                    = {Queueing Systems Volume {II}: {C}omputer Applications},
  Author                   = {L. Kleinrock},
  Publisher                = {New York: Wiley},
  Year                     = {1976}
}

@Article{kleinrock1975packet,
  Title                    = {Packet switching in radio channels: {Part I}--carrier sense multiple-access modes and their throughput-delay characteristics},
  Author                   = {Kleinrock, Leonard and Tobagi, Fouad A},
  Journal                  = {{IEEE} Trans. Commun.},
  Year                     = {1975},

  Month                    = {Dec.},
  Number                   = {12},
  Pages                    = {1400--1416},
  Volume                   = {23}
}

@Article{kobayashi2011training,
  Title                    = {Training and feedback optimization for multiuser {MIMO} downlink},
  Author                   = {Kobayashi, Mari and Jindal, Nihar and Caire, Giuseppe},
  Journal                  = {{IEEE} Trans. Commun},
  Year                     = {2011},

  Month                    = {Aug.},
  Number                   = {8},
  Pages                    = {2228--2240},
  Volume                   = {59}
}

@InProceedings{kulkarni2014coverage,
  Title                    = {Coverage and rate trends in dense urban mmwave cellular networks},
  Author                   = {Kulkarni, Mandar N and Singh, Sarabjot and Andrews, Jeffrey G},
  Booktitle                = {Proc. {IEEE} Global Communications Conference (GLOBECOM)},
  Year                     = {2014},
  Pages                    = {3809--3814}
}

@Article{kyasanur2009capacity,
  Title                    = {Capacity of multichannel wireless networks under the protocol model},
  Author                   = {Kyasanur, Pradeep and Vaidya, Nitin H},
  Journal                  = {{IEEE/ACM} Trans. Netw.},
  Year                     = {2009},

  Month                    = {Apr.},
  Number                   = {2},
  Pages                    = {515--527},
  Volume                   = {17}
}

@Article{Larsson2014massive,
  Title                    = {Massive {MIMO} for next generation wireless systems},
  Author                   = {Larsson, Erik G and Edfors, Ove and Tufvesson, Fredrik and Marzetta, Thomas L},
  Journal                  = {{IEEE} Commun. Mag.},
  Year                     = {2014},

  Month                    = {Feb.},
  Number                   = {2},
  Pages                    = {186--195},
  Volume                   = {52},

  File                     = {#F#}
}

@InProceedings{le2010longest,
  Title                    = {Longest-queue-first scheduling under {SINR} interference model},
  Author                   = {Le, Long Bao and Modiano, Eytan and Joo, Changhee and Shroff, Ness B},
  Booktitle                = {Proc. {ACM} International Symposium on Mobile Ad hoc Networking and Computing (MobiHoc)},
  Year                     = {2010},
  Pages                    = {41--50}
}

@InProceedings{Li2014Coordniation,
  Title                    = {Coordination context-based spectrum sharing for {5G} millimeter-wave networks},
  Author                   = {G. Li and T. Irnich and and C. Shi},
  Booktitle                = {Proc. International Conference on Cognitive Radio Oriented Wireless Networks and Communications (CROWNCOM)},
  Year                     = {2014},
  Month                    = {Jun.},
  Pages                    = {32--38}
}

@Article{Li:15,
  Title                    = {Joint Precoding and Load Balancing Optimization for Energy-Effiicient Heterogeneous Networks},
  Author                   = {J. Li and E. Bj\"{o}rnson and T. Svensson and T. Eriksson and M. Debbah},
  Journal                  = {IEEE Trans. Wireless Commun.},
  Year                     = {2015},

  Month                    = {Jun.},
  Number                   = {10},
  Pages                    = {5810-5822},
  Volume                   = {14}
}

@InProceedings{li2013anchor,
  Title                    = {Anchor-booster based heterogeneous networks with mmwave capable booster cells},
  Author                   = {Li, Qian Clara and Niu, Huaning and Wu, Geng and Hu, Rose Qingyang},
  Booktitle                = {Proc. {IEEE} Globecom Workshops},
  Year                     = {2013},
  Pages                    = {93--98}
}

@Article{liang2015wireless,
  Title                    = {Wireless network virtualization: {A} survey, some research issues and challenges},
  Author                   = {Liang, Chengchao and Yu, F Richard},
  Journal                  = {{IEEE} Commun. Surveys Tuts.},
  Year                     = {2015},

  Month                    = {First Quarter},
  Number                   = {1},
  Pages                    = {358--380},
  Volume                   = {17}
}

@InProceedings{liu2003capacity,
  Title                    = {On the capacity of hybrid wireless networks},
  Author                   = {Liu, Benyuan and Liu, Zhe and Towsley, Don},
  Booktitle                = {Proc. {IEEE} International Conference on Computer Communications (INFOCOM)},
  Year                     = {2003},
  Pages                    = {1543--1552},
  Volume                   = {2}
}

@InProceedings{liu2004study,
  Title                    = {A study of the coverage of large-scale sensor networks},
  Author                   = {Liu, Benyuan and Towsley, Don},
  Booktitle                = {Proc. {IEEE} International Conference on Mobile Ad hoc and Sensor Systems (MASS)},
  Year                     = {2004},
  Pages                    = {475--483}
}

@InProceedings{liu2009design,
  Title                    = {Design and analysis of {LTE} physical downlink control channel},
  Author                   = {J. Liu and R. Love and K. Stewart and M. Buckley},
  Booktitle                = {Proc {IEEE} Vehicular Technology Conference (VTC Spring)},
  Year                     = {2009},
  Pages                    = {1--5}
}

@Article{Lo2011Survey,
  Title                    = {A Survey of Common Control Channel Design in Cognitive Radio Networks},
  Author                   = {B.F. Lo},
  Journal                  = {Physical Communication (Elsevier)},
  Year                     = {2011},

  Month                    = {Mar.},
  Number                   = {1},
  Pages                    = {26--39},
  Volume                   = {4},

  File                     = {#F#}
}

@Article{lozin2008polynomial,
  Title                    = {A polynomial algorithm to find an independent set of maximum weight in a fork-free graph},
  Author                   = {Lozin, Vadim V and Milani{\v{c}}, Martin},
  Journal                  = {Journal of Discrete Algorithms},
  Year                     = {2008},
  Number                   = {4},
  Pages                    = {595--604},
  Volume                   = {6},

  Publisher                = {Elsevier}
}

@Article{lu2012modeling,
  Title                    = {Modeling the Impact of Human Blockers in Millimeter Wave Radio Links},
  Author                   = {Lu, Jonathan and Steinbach, Daniel and Cabrol, Patrick and Pietraski, Philip},
  Journal                  = {{ZTE} Commun. Mag.},
  Year                     = {2012},

  Month                    = {Jan.},
  Number                   = {4},
  Pages                    = {23--28},
  Volume                   = {10}
}

@Article{Lu2014Overview,
  Title                    = {An Overview of Massive {MIMO}: {B}enefits and Challenges},
  Author                   = {L. Lu and G. Y. Li and A. L. Swindlehurst and A. Ashikhmin and R. Zhang},
  Journal                  = {{IEEE} J. Sel. Top. Sign. Proces.},
  Year                     = {2014},

  Month                    = {Oct.},
  Number                   = {5},
  Pages                    = {742--758},
  Volume                   = {8},

  File                     = {#F#}
}

@InProceedings{lu2015stochastic,
  Title                    = {Stochastic geometry modeling of {mmWave} cellular networks: {A}nalysis and experimental validation},
  Author                   = {Lu, Wei and {Di Renzo}, Marco},
  Booktitle                = {Proc. {IEEE} International Workshop on Measurements Networking},
  Year                     = {2015},
  Month                    = {Oct.},
  Pages                    = {1-4},

  Doi                      = {10.1109/IWMN.2015.7322991}
}

@Article{magistretti2014802,
  Title                    = {802.11ec: {C}ollision avoidance without control messages},
  Author                   = {Magistretti, Eugenio and Gurewitz, Omer and Knightly, Edward W},
  Journal                  = {{IEEE/ACM} Trans. Netw.},
  Year                     = {2014},

  Month                    = {Dec.},
  Number                   = {6},
  Pages                    = {1845--1858},
  Volume                   = {22}
}

@Article{malone2007modeling,
  Title                    = {Modeling the 802.11 distributed coordination function in nonsaturated heterogeneous conditions},
  Author                   = {Malone, David and Duffy, Ken and Leith, Doug},
  Journal                  = {{IEEE/ACM} Trans. Netw.},
  Year                     = {2007},

  Month                    = {Feb.},
  Number                   = {1},
  Pages                    = {159--172},
  Volume                   = {15}
}

@Article{marina2010topology,
  Title                    = {A topology control approach for utilizing multiple channels in multi-radio wireless mesh networks},
  Author                   = {Marina, Mahesh K and Das, Samir R and Subramanian, Anand Prabhu},
  Journal                  = {Computer Networks},
  Year                     = {2010},

  Month                    = {Feb.},
  Number                   = {2},
  Pages                    = {241--256},
  Volume                   = {54}
}

@Article{Marler2004Survey,
  Title                    = {Survey of multi-objective optimization methods for engineering},
  Author                   = {R. T. Marler and J. S. Arora},
  Journal                  = {Struct. Multidiscip. O.},
  Year                     = {2004},

  Month                    = {Apr.},
  Number                   = {6},
  Pages                    = {369--395},
  Volume                   = {26},

  File                     = {#F#}
}

@Article{marzetta2010noncooperative,
  Title                    = {Noncooperative cellular wireless with unlimited numbers of base station antennas},
  Author                   = {Marzetta, Thomas L},
  Journal                  = {{IEEE} Trans. Wireless Commun.},
  Year                     = {2010},

  Month                    = {Nov.},
  Number                   = {11},
  Pages                    = {3590--3600},
  Volume                   = {9},

  Publisher                = {IEEE}
}

@Article{mukherjee2014principles,
  Title                    = {Principles of physical layer security in multiuser wireless networks: {A} survey},
  Author                   = {Mukherjee, Arjun and Fakoorian, S Ali and Huang, Jing and Swindlehurst, A Lee and others},
  Journal                  = {{IEEE} Commun. Surveys Tuts.},
  Year                     = {2014},

  Month                    = {Third Quarter},
  Number                   = {3},
  Pages                    = {1550--1573},
  Volume                   = {16}
}

@Article{nakamura2013trends,
  Title                    = {Trends in small cell enhancements in {LTE} advanced},
  Author                   = {Nakamura, Takehiro and Nagata, Satoshi and Benjebbour, Anass and Kishiyama, Yoshihisa and Hai, Tang and Xiaodong, Shen and Ning, Yang and Nan, Li},
  Journal                  = {{IEEE} Commun. Mag.},
  Year                     = {2013},

  Month                    = {Feb.},
  Number                   = {2},
  Pages                    = {98--105},
  Volume                   = {51}
}

@Article{Nam2014Joint,
  Title                    = {Joint spatial division and multiplexing: {O}pportunistic beamforming, user grouping and simplified downlink scheduling},
  Author                   = {J. Nam and A. Adhikary and J. Ahn and G. Caire},
  Journal                  = {{IEEE} J. Sel. Areas Commun.},
  Year                     = {2014},

  Month                    = {Oct.},
  Number                   = {5},
  Pages                    = {876--890},
  Volume                   = {8},

  File                     = {#F#}
}

@InProceedings{nandagopal2000achieving,
  Title                    = {Achieving {MAC} layer fairness in wireless packet networks},
  Author                   = {Nandagopal, Thyagarajan and Kim, Tae-Eun and Gao, Xia and Bharghavan, Vaduvur},
  Booktitle                = {Proc. {ACM} International Conference on Mobile Computing and Networking (MobiCom)},
  Year                     = {2000},
  Pages                    = {87--98}
}

@Article{nelson1985spatial,
  Title                    = {Spatial {TDMA}: {A} collision-free multihop channel access protocol},
  Author                   = {Nelson, Randolph and Kleinrock, Leonard},
  Journal                  = {{IEEE} Trans. Commun.},
  Year                     = {1985},

  Month                    = {Sept.},
  Number                   = {9},
  Pages                    = {934--944},
  Volume                   = {33}
}

@Article{ngo2013energy,
  Title                    = {Energy and spectral efficiency of very large multiuser {MIMO} systems},
  Author                   = {Ngo, Hien Quoc and Larsson, Erik G and Marzetta, Thomas L},
  Journal                  = {{IEEE} Trans. Commun.},
  Year                     = {2013},

  Month                    = {Feb.},
  Number                   = {4},
  Pages                    = {1436--1449},
  Volume                   = {61}
}

@Article{Nitsche2014IEEE,
  Title                    = {{IEEE 802.11ad}: {D}irectional {60~GHz} communication for multi-{G}igabit-per-second {Wi-Fi}},
  Author                   = {Nitsche, Thomas and Cordeiro, Carlos and Flores, Adriana B and Knightly, Edward W and Perahia, Eldad and Widmer, Joerg C},
  Journal                  = {{IEEE} Commun. Mag.},
  Year                     = {2014},

  Month                    = {Dec.},
  Number                   = {12},
  Pages                    = {132--141},
  Volume                   = {52},

  File                     = {#F#}
}

@Article{niu2015exploiting,
  Title                    = {Exploiting Device-to-Device Communications in Joint Scheduling of Access and Backhaul for {mmWave} Small Cells},
  Author                   = {Niu, Yong and Gao, Chuhan and Li, Yong and Su, Li and Jin, Depeng and Vasilakos, Athanasios},
  Journal                  = {{IEEE} J. Sel. Areas Commun.},
  Year                     = {2015},

  Month                    = {Oct.},
  Number                   = {10},
  Pages                    = {2052--2069},
  Volume                   = {33}
}

@Article{Niu2015Survey,
  Title                    = {A survey of millimeter wave communications {(mmWave)} for {5G}: {O}pportunities and challenges},
  Author                   = {Niu, Yong and Li, Yong and Jin, Depeng and Su, Li and Vasilakos, Athanasios},
  Journal                  = {Wireless Networks},
  Year                     = {2015},

  Month                    = {Apr.},
  Pages                    = {1--20}
}

@Article{Niu2015Blockage,
  Title                    = {Blockage Robust and Efficient Scheduling for Directional {mmWave WPANs}},
  Author                   = {Y. Niu and Y. Li and D. Jin and L. Su and D. Wu},
  Journal                  = {{IEEE} Trans. Veh. Technol.},
  Year                     = {2015},

  Month                    = {Feb.},
  Number                   = {2},
  Pages                    = {728--742},
  Volume                   = {64}
}

@Article{ntranos2015cellular,
  Title                    = {Cellular interference alignment},
  Author                   = {Ntranos, Vasilis and Maddah-Ali, Mohammad Ali and Caire, Giuseppe},
  Journal                  = {{IEEE} Trans. Inf. Theory},
  Year                     = {2015},

  Month                    = {Mar.},
  Number                   = {3},
  Pages                    = {1194--1217},
  Volume                   = {61}
}

@Article{Ofcom1,
  Title                    = {Spectrum above {6GHz} for future mobile communications},
  Author                   = {{Ofcom}},
  Year                     = {2015},

  Month                    = {Feb.},

  Url                      = {http://stakeholders.ofcom.org.uk/binaries/consultations/above-6ghz/summary/spectrum_above_6_GHz_CFI.pdf}
}

@article{gai2012combinatorial,
  title={Combinatorial network optimization with unknown variables: {Multi-armed} bandits with linear rewards and individual observations},
  author={Gai, Yi and Krishnamachari, Bhaskar and Jain, Rahul},
  journal={IEEE/ACM Trans. Netw.},
  volume={20},
  number={5},
  pages={1466--1478},
  year={2012},
  month={Oct.}
}

@article{Razaviyayn_BCD_12,
	Author = {Razaviyayn, Meisam and Hong, Mingyi and Luo, Zhi-Quan},
	Journal = {SIAM Journal on Optimization},
    volume={23},
    number={2},
    pages={1126--1153},	
    month={June},
	Title = {A Unified Convergence Analysis of Block Successive Minimization Methods for Nonsmooth Optimization},
	Year = {2013}
}

@Article{osseiran2014scenarios,
  Title                    = {Scenarios for {5G} mobile and wireless communications: the vision of the {METIS} project},
  Author                   = {Osseiran, Afif and Boccardi, Federico and Braun, Volker and Kusume, Katsutoshi and Marsch, Patrick and Maternia, Michal and Queseth, Olav and Schellmann, Malte and Schotten, Hans and Taoka, Hidekazu and others},
  Journal                  = {{IEEE} Commun. Mag.},
  Year                     = {2014},

  Month                    = {May},
  Number                   = {5},
  Pages                    = {26--35},
  Volume                   = {52}
}

@Article{Park2007Short,
  Title                    = {Short-range wireless communications for Next-Generation Networks: {UWB}, 60 {GHz} millimeter-wave {WPAN}, and {ZigBee}},
  Author                   = {C. Park and T.S. Rappaport},
  Journal                  = {{IEEE} Wireless Commun.},
  Year                     = {2007},

  Month                    = {Aug.},
  Number                   = {4},
  Pages                    = {70--78},
  Volume                   = {14},

  File                     = {#F#}
}

@Article{park2015TractableResource,
  Title                    = {Tractable Resource Management in Millimeter-Wave Overlaid Ultra-Dense Cellular Networks},
  Author                   = {Park, Jihong and Kim, Seong-Lyun and Zander, Jens},
  Journal                  = {arXiv preprint arXiv:1507.04658},
  Year                     = {2015}
}

@Article{Park2009Analysis,
  Title                    = {Analysis on Spatial Reuse and Interference in 60-{GHz} Wireless Networks},
  Author                   = {M. Park and P. Gopalakrishnan},
  Journal                  = {{IEEE} J. Sel. Areas Commun.},
  Year                     = {2009},

  Month                    = {Oct.},
  Number                   = {8},
  Pages                    = {1443--1452},
  Volume                   = {27},

  File                     = {#F#}
}

@InProceedings{park2009generalized,
  Title                    = {A generalized {Markov} chain model for effective analysis of slotted {IEEE 802.15.4}},
  Author                   = {Park, Pangun and Di Marco, Piergiuseppe and Soldati, Pablo and Fischione, Carlo and Johansson, Karl Henrik},
  Booktitle                = {Proc. {IEEE} Mobile Adhoc and Sensor Systems (MASS)},
  Year                     = {2009},
  Pages                    = {130--139}
}

@Article{pollin2008performance,
  Title                    = {Performance analysis of slotted carrier sense {IEEE 802.15.4} medium access layer},
  Author                   = {Pollin, Sofie and Ergen, Mustafa and Ergen, Sinem and Bougard, Bruno and Der Perre, L and Moerman, Ingrid and Bahai, Ahmad and Varaiya, Pravin and Catthoor, Francky},
  Journal                  = {{IEEE} Trans. Wireless Commun.},
  Year                     = {2008},

  Month                    = {Sept.},
  Number                   = {9},
  Pages                    = {3359--3371},
  Volume                   = {7}
}

@Article{Dana2007Information,
  Title                    = {Information Theory of Wideband Communications},
  Author                   = {Dana Porrat},
  Journal                  = {{IEEE} Commun. Surveys Tuts.},
  Year                     = {2007},

  Month                    = {Second Quarter},
  Number                   = {2},
  Pages                    = {2--16},
  Volume                   = {9}
}

@Article{pyo2009throughput,
  Title                    = {Throughput analysis and improvement of hybrid multiple access in {IEEE 802.15.3c} mm-wave {WPAN}},
  Author                   = {Pyo, Chang Woo and Harada, Hiroshi},
  Journal                  = {{IEEE} J. Sel. Areas Commun.},
  Year                     = {2009},

  Month                    = {Oct.},
  Number                   = {8},
  Pages                    = {1414--1424},
  Volume                   = {27}
}

@Article{Qiao2011Enabling,
  Title                    = {Enabling multi-hop concurrent transmissions in 60 {GHz} wireless personal area networks},
  Author                   = {J. Qiao and L. Cai and X. Shen and J. Mark},
  Journal                  = {{IEEE} Trans. Wireless Commun.},
  Year                     = {2011},

  Month                    = {Nov.},
  Number                   = {11},
  Pages                    = {3824--3833},
  Volume                   = {10},

  File                     = {#F#}
}

@InProceedings{Qiao2012STDMA,
  Title                    = {{STDMA}-based scheduling algorithm for concurrent transmissions in directional millimeter wave networks},
  Author                   = {J. Qiao and L. X. Cai and X. Shen and J. Mark},
  Booktitle                = {Proc. {IEEE} International Conference on Communications (ICC)},
  Year                     = {2012},
  Pages                    = {5221--5225}
}

@Article{Qiao2015D2D,
  Title                    = {Enabling device-to-device communications in millimeter-wave {(5G)} cellular networks},
  Author                   = {J. Qiao and X. Shen and J. Mark and Q. Shen and Y. He and L. Lei},
  Journal                  = {{IEEE} Commun. Mag.},
  Year                     = {2015},

  Month                    = {Jan.},
  Number                   = {1},
  Pages                    = {209--215},
  Volume                   = {53}
}

@Article{Raghavan2007Capacity,
  Title                    = {Capacity of Sparse Multipath Channels in the Ultra-Wideband Regime},
  Author                   = {V. Raghavan and Gautham Hariharan and Akbar M. Sayeed},
  Journal                  = {{IEEE} J. Sel. Topics Signal Proc.},
  Year                     = {2007},

  Month                    = {Oct.},
  Number                   = {3},
  Pages                    = {357--371},
  Volume                   = {1}
}

@Article{Ramanathan2005Adhoc,
  Title                    = {Ad hoc networking with directional antennas: {A} complete system solution},
  Author                   = {R. Ramanathan and J. Redi and C. Santivanez and D. Wiggins and S. Polit},
  Journal                  = {{IEEE} J. Sel. Areas Commun.},
  Year                     = {2005},

  Month                    = {Mar.},
  Number                   = {3},
  Pages                    = {496--506},
  Volume                   = {23},

  File                     = {#F#}
}

@InProceedings{ramanathan1997unified,
  Title                    = {A unified framework and algorithm for {(T/F/C) DMA} channel assignment in wireless networks},
  Author                   = {Ramanathan, S},
  Booktitle                = {Proc. {IEEE} International Conference on Computer Communications (INFOCOM)},
  Year                     = {1997},
  Pages                    = {900--907}
}

@Article{Rangan2014Millimeter,
  Title                    = {Millimeter Wave Cellular Wireless Networks: {P}otentials and Challenges},
  Author                   = {S. Rangan and T.S. Rappaport and E. Erkip},
  Journal                  = {Proc. {IEEE}},
  Year                     = {2014},

  Month                    = {Mar.},
  Number                   = {3},
  Pages                    = {366--385},
  Volume                   = {102},

  File                     = {#F#}
}

@Article{Rappaport2013Millimeter,
  Title                    = {Millimeter Wave Mobile Communications for {5G} Cellular: {I}t Will Work!},
  Author                   = {T.S. Rappaport and S. Sun and R. Mayzus and H. Zhao and Y. Azar and K. Wang and G. Wong and J. Schulz and M. Samimi and F. Gutierrez},
  Journal                  = {{IEEE} Access},
  Year                     = {2013},

  Month                    = {May},
  Pages                    = {335--349},
  Volume                   = {1},

  File                     = {#F#}
}

@Book{rappaport2002wireless,
  Title                    = {Wireless communications: {P}rinciples and practice},
  Author                   = {Rappaport, Theodore S},
  Publisher                = {Prentice Hall PTR New Jersey},
  Year                     = {2002}
}

@Book{Rappaport2014mmWaveBook,
  Title                    = {Millimeter Wave Wireless Communications},
  Author                   = {Rappaport, Theodore S and Heath, Robert and Daniels, Robert C and Murdock, James N},
  Publisher                = {Pearson Education},
  Year                     = {2014}
}

@Article{Rappaport2015wideband,
  Title                    = {Wideband Millimeter-Wave Propagation Measurements and Channel Models for Future Wireless Communication System Design},
  Author                   = {Theodore S. Rappaport and George R. MacCartney and Mathew K. Samimi and Shu Sun},
  Journal                  = {{IEEE} Trans. Commun.},
  Year                     = {2015},

  Month                    = {Sept.},
  Number                   = {9},
  Pages                    = {3029--3056},
  Volume                   = {63}
}

@Article{rashid1998joint,
  Title                    = {Joint optimal power control and beamforming in wireless networks using antenna arrays},
  Author                   = {Rashid-Farrokhi, Farrokh and Tassiulas, Leandros and Liu, KJ},
  Journal                  = {{IEEE} Trans. Commun.},
  Year                     = {1998},

  Month                    = {Oct.},
  Number                   = {10},
  Pages                    = {1313--1324},
  Volume                   = {46}
}

@Article{Rebatoy2016Potential,
  Title                    = {The Potential of Resource Sharing in {5G} Millimeter-Wave Bands},
  Author                   = {Mattia Rebatoy and Marco Mezzavilla and Sundeep Rangan and Michele Zorzi},
  Journal                  = {arXiv preprint arXiv:1602.07732},
  Year                     = {206}
}

@Article{rhee2008z,
  Title                    = {{Z-MAC}: {A} hybrid {MAC} for wireless sensor networks},
  Author                   = {Rhee, Injong and Warrier, Ajit and Aia, Mahesh and Min, Jeongki and Sichitiu, Mihail L},
  Journal                  = {{IEEE/ACM} Trans. Netw.},
  Year                     = {2008},

  Month                    = {Jun.},
  Number                   = {3},
  Pages                    = {511--524},
  Volume                   = {16}
}

@InProceedings{rhee2006drand,
  Title                    = {DRAND: {D}istributed randomized {TDMA} scheduling for wireless ad-hoc networks},
  Author                   = {Rhee, Injong and Warrier, Ajit and Min, Jeongki and Xu, Lisong},
  Booktitle                = {Proc. {ACM} international symposium on Mobile ad hoc networking and computing (MobiHoc)},
  Year                     = {2006},
  Organization             = {ACM},
  Pages                    = {190--201}
}

@Article{rios1985hybrid,
  Title                    = {A hybrid multiple-access protocol for data and voice-packet over local area networks},
  Author                   = {Rios, Miguel and Georganas, Nicolas D},
  Journal                  = {{IEEE} Trans. Comput.},
  Year                     = {1985},

  Month                    = {Jan.},
  Number                   = {1},
  Pages                    = {90--94},
  Volume                   = {100}
}

@InCollection{robbins1985some,
  Title                    = {Some aspects of the sequential design of experiments},
  Author                   = {Robbins, Herbert},
  Booktitle                = {Herbert Robbins Selected Papers},
  Publisher                = {Springer},
  Year                     = {1985},
  Pages                    = {169--177}
}

@Article{Roh2014Millimeter,
  Title                    = {Millimeter-wave beamforming as an enabling technology for {5G} cellular communications: {Teoretical} feasibility and prototype results},
  Author                   = {W. Roh and J.Y. Seol and J. Park and B. Lee and J. Lee and Y. Kim and J. Cho and K. Cheun and F. Aryanfar},
  Journal                  = {{IEEE} Commun. Mag.},
  Year                     = {2014},

  Month                    = {Feb.},
  Number                   = {2},
  Pages                    = {106--113},
  Volume                   = {52},

  File                     = {#F#}
}

@Article{Salem2010Opportunities,
  Title                    = {Opportunities and Challenges in {OFDMA}-Based Cellular Relay Networks: {A} Radio Resource Management Perspective},
  Author                   = {M. Salem and A. Adinoyi and H. Yanikomeroglu and D. Falconer},
  Journal                  = {{IEEE} Trans. Veh. Technol.},
  Year                     = {2010},

  Month                    = {Jun.},
  Number                   = {5},
  Pages                    = {2496--2510},
  Volume                   = {59},

  File                     = {#F#}
}

@article{phan2009spectrum,
  title={Spectrum sharing in wireless networks via {QoS}-aware secondary multicast beamforming},
  author={Phan, Khoa T and Vorobyov, Sergiy A and Sidiropoulos, Nicholas D and Tellambura, Chintha},
  journal={{IEEE} Trans. Signal Process.},
  volume={57},
  number={6},
  pages={2323--2335},
  year={2009},
  month={Jun.}
}

@Article{sayeed2002deconstructing,
  Title                    = {Deconstructing multiantenna fading channels},
  Author                   = {Sayeed, Akbar M},
  Journal                  = {{IEEE} Trans. Signal Process.},
  Year                     = {2002},
  Month                    = {Oct.},
  Number                   = {10},
  Pages                    = {2563--2579},
  Volume                   = {50}
}

@Article{schubert2004solution,
  Title                    = {Solution of the multiuser downlink beamforming problem with individual {SINR} constraints},
  Author                   = {Schubert, Martin and Boche, Holger},
  Journal                  = {{IEEE} Trans. Veh. Technol.},
  Year                     = {2004},

  Month                    = {Jan.},
  Number                   = {1},
  Pages                    = {18--28},
  Volume                   = {53}
}

@Article{seifi2015media,
  Title                    = {Media-Based {MIMO}: {A} New Frontier in Wireless Communications},
  Author                   = {Seifi, Ehsan and Atamanesh, Mehran and Khandani, Amir K},
  Journal                  = {arXiv preprint arXiv:1507.07516},
  Year                     = {2015}
}

@Book{sesia2009lte,
  Title                    = {{LTE}: {T}he UMTS long term evolution},
  Author                   = {Sesia, Stefania and Toufik, Issam and Baker, Matthew},
  Publisher                = {Wiley Online Library},
  Year                     = {2009}
}

@Article{sharif2005capacity,
  Title                    = {On the capacity of {MIMO} broadcast channels with partial side information},
  Author                   = {Sharif, Masoud and Hassibi, Babak},
  Journal                  = {{IEEE} Trans. Inform. Theory},
  Year                     = {2005},

  Month                    = {Feb.},
  Number                   = {2},
  Pages                    = {506--522},
  Volume                   = {51}
}

@Article{shearer1983note,
  Title                    = {A note on the independence number of triangle-free graphs},
  Author                   = {Shearer, James B},
  Journal                  = {Discrete Mathematics},
  Year                     = {1983},
  Number                   = {1},
  Pages                    = {83--87},
  Volume                   = {46}
}

@PhdThesis{Shokri2015Licentiate,
  Title                    = {Fundamentals of Medium Access Control Design for Millimeter Wave Networks},
  Author                   = {Hossein Shokri-Ghadikolaei},
  School                   = {KTH, Royal Institute of Technology},
  Year                     = {2015},
  Month                    = {Sept.},
  Type                     = {Licentiate Thesis}
}

@Article{shokri2016Spectrum,
  Title                    = {Spectrum sharing in {mmWave} cellular networks via cell association, coordination, and beamforming},
  Author                   = {Shokri-Ghadikolaei, Hossein and Boccardi, Federico and Fischione, Carlo and Fodor, Gabor and Zorzi, Michele},
  Journal                  = {{IEEE} J. Sel. Areas Commun.},
  Year                     = {2016},

  Month                    = {Nov.},
  Number                   = {11},
  Pages                    = {2902--2917},
  Volume                   = {34}
}

@article{yuceer2002discrete,
  title={Discrete convexity: convexity for functions defined on discrete spaces},
  author={Y{\"u}ceer, {\"U}mit},
  journal={Discrete Applied Mathematics},
  volume={119},
  number={3},
  pages={297--304},
  year={2002},
  publisher={Elsevier}
}

@book{murota2003discrete,
  title={Discrete convex analysis},
  author={Murota, Kazuo},
  year={2003},
  publisher={SIAM}
}

@article{xu2013block,
  title={A block coordinate descent method for regularized multiconvex optimization with applications to nonnegative tensor factorization and completion},
  author={Xu, Yangyang and Yin, Wotao},
  journal={SIAM Journal on Imaging Sciences},
  volume={6},
  number={3},
  pages={1758--1789},
  year={2013},
  publisher={SIAM}
}

@inproceedings{karimi2016linear,
  title={Linear convergence of gradient and proximal-gradient methods under the polyak-{\l}ojasiewicz condition},
  author={Karimi, Hamed and Nutini, Julie and Schmidt, Mark},
  booktitle={Joint European Conference on Machine Learning and Knowledge Discovery in Databases},
  pages={795--811},
  year={2016},
  organization={Springer}
}

@Article{Shokri2015Transitional,
  Title                    = {The transitional behavior of interference in millimeter wave networks and its impact on medium access control},
  Author                   = {Hossein S. Ghadikolaei and Carlo Fischione},
  Journal                  = {{IEEE} Transactions on Communications},
  Year                     = {2016},
  Month                    = {Feb.},
  Number                   = {2},
  Pages                    = {723--740},
  Volume                   = {62}
}

@InProceedings{shokri2015MillimeterGlobecom,
  Title                    = {Millimeter Wave Ad Hoc Networks: {N}oise-limited or Interference-limited?},
  Author                   = {Hossein Shokri-Ghadikolaei and Carlo Fischione},
  Booktitle                = {Proc. {IEEE} Global Communications Conference (GLOBECOM) Workshops},
  Year                     = {2015}
}

@Article{shokri2015mmWavecellular,
  Title                    = {Millimeter wave cellular networks: {A} {MAC} layer perspective},
  Author                   = {H. Shokri-Ghadikolaei and C. Fischione and G. Fodor and P. Popovski and M. Zorzi},
  Journal                  = {{IEEE} Transactions on Communications},
  Year                     = {2015},

  Month                    = {Oct.},
  Number                   = {10},
  Pages                    = {3437--3458},
  Volume                   = {63}
}

@article{Jiang2019LowLatency,
  title={Low-latency networking: {W}here latency lurks and how to tame it},
  author={X. Jiang and H. S. Ghadikolaei and G. Fodor and E. Modiano and Z. Pang and M. Zorzi and C. Fischione},
  journal={Proc. {IEEE}},
  volume = {107},
  number = {2},
  pages = {280--306},
  month={Feb.},
  year = {2019},
}

@article{Bottou2018SIAM,
author = {Bottou, L. and Curtis, F. and Nocedal, J.},
title = {Optimization Methods for Large-Scale Machine Learning},
journal = {SIAM Review},
volume = {60},
number = {2},
pages = {223-311},
year = {2018},
}

@InProceedings{Shokri2016OntheAccuracy,
  Title                    = {On the Accuracy of Interference Models in Wireless Communications},
  Author                   = {Hossein Shokri-Ghadikolaei and Carlo Fischione and Eytan Modiano},
  Booktitle                = {Proc. {IEEE} International Conference on Communications (ICC)},
  Year                     = {2016}
}

@TechReport{Shokri2015ConflictGraph,
  Title                    = {Characterizing the conflict graph of millimeter wave networks},
  Author                   = {Hossein Shokri-Ghadikolaei and Carlo Fischione and Eytan Modiano},
  Institution              = {KTH Royal Institute of Technology},
  Year                     = {2015},
  Month                    = {Nov.},
  Note                     = {available upon request}
}

@Article{Shokri2015mmWaveWPAN,
  Title                    = {Design Aspects of Short Range Millimeter Wave Wireless Networks: {A} {MAC} Layer Perspective},
  Author                   = {Hossein Shokri-Ghadikolaei and Carlo Fischione and Petar Popovski and Michele Zorzi},
  Journal                  = {{IEEE} Netw.},
  Year                     = {2015},
  Note                     = {Accepted, To appear}
}

@InProceedings{Shokri2015Beam,
  Title                    = {Beam-searching and Transmission Scheduling in Millimeter Wave Communications},
  Author                   = {Hossein Shokri-Ghadikolaei and Lazaros Gkatzikis and Carlo Fischione},
  Booktitle                = {Proc. {IEEE} International Conference on Communications (ICC)},
  Year                     = {2015},
  Pages                    = {1292--1297}
}

@TechReport{Shokri2015WhatIs,
  Title                    = {What Is the Right Interference Model in Millimeter Wave Networks?},
  Author                   = {Hossein Shokri-Ghadikolaei and Xiaolin Jiang and Carlo Fischione and Pang Zhibo},
  Institution              = {KTH Royal Institute of Technology},
  Year                     = {2015},
  Month                    = {Nov.},

  Url                      = {http://www.kth.se/social/files/564f32e4f276547c6f6b80a3/manuscript-v04.pdf}
}

@TechReport{Shokri2015interplay,
  Title                    = {The interplay between beam training and association in millimeter wave networks},
  Author                   = {Hossein Shokri-Ghadikolaei and Yuzhe Xu and Carlo Fischione},
  Institution              = {KTH Royal Institute of Technology},
  Year                     = {2015},
  Month                    = {Jul.},
  Note                     = {available upon request}
}

@Article{Singh2015TractableModel,
  Title                    = {Tractable Model for Rate in Self-Backhauled Millimeter Wave Cellular Networks},
  Author                   = {Sarabjot Singh and Mandar N. Kulkarni and Amitava Ghosh and Jeffrey G. Andrews},
  Journal                  = {{IEEE} J. Sel. Areas Commun.},
  Year                     = {2015},

  Month                    = {Oct.},
  Number                   = {10},
  Pages                    = {2196--2211},
  Volume                   = {33}
}

@InProceedings{Singh2010Distributed,
  Title                    = {Distributed coordination with deaf neighbors: {E}fficient medium access for 60{GHz} mesh networks},
  Author                   = {S. Singh and M. Mudumbai and U. Madhow},
  Booktitle                = {Proc. {IEEE} International Conference on Computer Communications (INFOCOM)},
  Year                     = {2010},
  Pages                    = {1--9}
}

@Article{Singh2011Interference,
  Title                    = {Interference analysis for highly directional 60-{GHz} mesh networks: {T}he case for rethinking medium access control},
  Author                   = {S. Singh and R. Mudumbai and U. Madhow},
  Journal                  = {{IEEE/ACM} Trans. Netw.},
  Year                     = {2011},

  Month                    = {Oct.},
  Number                   = {5},
  Pages                    = {1513--1527},
  Volume                   = {19},

  File                     = {#F#}
}

@Article{Singh2009Blockage,
  Title                    = {Blockage and Directivity in 60 {GHz} Wireless Personal Area Networks: {F}rom Cross-Layer Model to Multihop {MAC} Design},
  Author                   = {S. Singh and F. Ziliotto and U. Madhow and E.M. Belding and M. Rodwell},
  Journal                  = {{IEEE} J. Sel. Areas Commun.},
  Year                     = {2009},

  Month                    = {Oct.},
  Number                   = {8},
  Pages                    = {1400--1413},
  Volume                   = {27},

  File                     = {#F#}
}

@InProceedings{Son2012on,
  Title                    = {On frame-based scheduling for directional {mmWave} {WPANs}},
  Author                   = {I.K. Son and S. Mao and M.X. Gong and Y. Li},
  Booktitle                = {Proc. {IEEE} International Conference on Computer Communications (INFOCOM)},
  Year                     = {2012},
  Pages                    = {2149--2157}
}

@InProceedings{son2012frame,
  Title                    = {On frame-based scheduling for directional {mmWave} {WPANs}},
  Author                   = {Son, In Keun and Mao, Shiwen and Gong, Michelle X and Li, Yihan},
  Booktitle                = {Proc. {IEEE} International Conference on Computer Communications (INFOCOM)},
  Year                     = {2012},
  Pages                    = {2149--2157}
}

@Article{sousa1990optimum,
  Title                    = {Optimum transmission ranges in a direct-sequence spread-spectrum multihop packet radio network},
  Author                   = {Sousa, Elvino S and Silvester, John and others},
  Journal                  = {Selected Areas in Communications, IEEE Journal on},
  Year                     = {1990},
  Number                   = {5},
  Pages                    = {762--771},
  Volume                   = {8}
}

@Article{springer1966distribution,
  Title                    = {The distribution of products of independent random variables},
  Author                   = {Springer, MD and Thompson, WE},
  Journal                  = {{SIAM} Journal on Applied Mathematics},
  Year                     = {1966},

  Month                    = {May},
  Number                   = {3},
  Pages                    = {511--526},
  Volume                   = {14}
}

@Article{srinivasa2010distance,
  Title                    = {Distance distributions in finite uniformly random networks: {T}heory and applications},
  Author                   = {Srinivasa, Sunil and Haenggi, Martin},
  Journal                  = {{IEEE} Trans. Veh. Technol.},
  Year                     = {2010},

  Month                    = {Feb.},
  Number                   = {2},
  Pages                    = {940--949},
  Volume                   = {59}
}

@Book{srivastava2001series,
  Title                    = {Series associated with the zeta and related functions},
  Author                   = {Srivastava, Hari M and Junesang, Choi},
  Publisher                = {Springer Science \& Business Media},
  Year                     = {2001},
  Volume                   = {530}
}

@Book{stoyan1987stochastic,
  Title                    = {Stochastic geometry and its applications},
  Author                   = {Stoyan, Dietrich and Kendall, Wilfrid S and Mecke, Joseph and Ruschendorf, L},
  Publisher                = {Wiley New York},
  Year                     = {1987},
  Volume                   = {2}
}

@Article{Sum2009virtual,
  Title                    = {Virtual Time-Slot Allocation Scheme for Throughput Enhancement in a Millimeter-Wave Multi-{Gbps} {WPAN} System},
  Author                   = {C. Sum and Z. Lan and R. Funada and J. Wang and T. Baykas and M. A. Rahman and H. Harada},
  Journal                  = {{IEEE} J. Sel. Areas Commun.},
  Year                     = {2009},

  Month                    = {Oct.},
  Number                   = {8},
  Pages                    = {1379--1389},
  Volume                   = {27}
}

@InProceedings{sun2014millimeter,
  Title                    = {Millimeter wave multi-beam antenna combining for {5G} cellular link improvement in {New York City}},
  Author                   = {Sun, Shu and MacCartney, George R and Samimi, Mathew K and Nie, Shuai and Rappaport, Theodore S},
  Booktitle                = {Proc. {IEEE} International Conference on Communications (ICC)},
  Year                     = {2014},
  Pages                    = {5468--5473}
}

@Article{Sun2014MIMO,
  Title                    = {{MIMO} for Millimeter Wave Wireless Communications: {B}eamforming, Spatial Multiplexing, or Both?},
  Author                   = {S. Sun and T. Rappapport and R. Heath and A. Nix and S. Rangan},
  Journal                  = {{IEEE} Commun. Mag.},
  Year                     = {2014},

  Month                    = {Dec.},
  Number                   = {12},
  Pages                    = {110--121},
  Volume                   = {52},

  File                     = {#F#}
}

@InProceedings{takai2001effects,
  Title                    = {Effects of wireless physical layer modeling in mobile ad hoc networks},
  Author                   = {Takai, Mineo and Martin, Jay and Bagrodia, Rajive},
  Booktitle                = {Proc. {ACM} International Symposium on Mobile ad hoc Networking \& Computing (MobiHoc)},
  Year                     = {2001},
  Pages                    = {87--94}
}

@Article{Taori2015Point,
  Title                    = {Point-to-multipoint in-band mmWave back-haul for 5G networks},
  Author                   = {R. Taori and A. Sridharan},
  Journal                  = {{IEEE} Commun. Mag.},
  Year                     = {2015},

  Month                    = {Jan},
  Number                   = {53},
  Pages                    = {195--201},
  Volume                   = {1}
}

@Article{thompson1956distribution,
  Title                    = {Distribution of distance to nth neighbour in a population of randomly distributed individuals},
  Author                   = {Thompson, HR},
  Journal                  = {Ecology},
  Year                     = {1956},
  Pages                    = {391--394}
}

@Article{thompson1933likelihood,
  Title                    = {On the likelihood that one unknown probability exceeds another in view of the evidence of two samples},
  Author                   = {Thompson, William R},
  Journal                  = {Biometrika},
  Year                     = {1933},
  Number                   = {3/4},
  Pages                    = {285--294},
  Volume                   = {25},

  Publisher                = {JSTOR}
}

@InProceedings{Thornburg2015mmWave,
  Title                    = {{MmWave} Ad Hoc Network Coverage and Capacity},
  Author                   = {A. Thornburg and T. Bai and R. Heath},
  Booktitle                = {Proc. {IEEE} International Conference on Communications (ICC)},
  Year                     = {2015},
  Pages                    = {1310--1315}
}

@TechReport{Toyoda2007Reference,
  Title                    = {Reference antenna model with sidelobe for {TG3c} evaluation},
  Author                   = {I. Toyoda and T. Seki and K. Iigusa and H. Sawada and Y. Fujita and A. Miura and N. Orihashi},
  Institution              = {IEEE 802.15-06-0474-00-003c},
  Year                     = {2007},
  Month                    = {Mar.}
}

@InProceedings{van2003adaptive,
  Title                    = {An adaptive energy-efficient {MAC} protocol for wireless sensor networks},
  Author                   = {Van Dam, Tijs and Langendoen, Koen},
  Booktitle                = {Proc. {ACM} international conference on mbedded networked sensor systems (SenSys)},
  Year                     = {2003},
  Pages                    = {171--180}
}

@Article{venkateswaran2010analog,
  Title                    = {Analog beamforming in {MIMO} communications with phase shift networks and online channel estimation},
  Author                   = {Venkateswaran, Vijay and Van der Veen, Alle-Jan},
  Journal                  = {{IEEE} Trans. Signal Process.},
  Year                     = {2010},
  Month                    = {Aug.},
  Number                   = {8},
  Pages                    = {4131--4143},
  Volume                   = {58}
}

@Article{verdu2002spectral,
  Title                    = {Spectral efficiency in the wideband regime},
  Author                   = {Verd{\'u}, Sergio},
  Journal                  = {{IEEE} Trans. Inf. Theory},
  Year                     = {2002},

  Month                    = {Jun.},
  Number                   = {6},
  Pages                    = {1319--1343},
  Volume                   = {48}
}

@Book{verdu1998multiuser,
  Title                    = {Multiuser detection},
  Author                   = {Verdu, Sergio},
  Publisher                = {Cambridge university press},
  Year                     = {1998}
}

@Article{vuran2007mac,
  Title                    = {{A-MAC}: {A}daptive medium access control for next generation wireless terminals},
  Author                   = {Vuran, Mehmet C and Akyildiz, Ian F},
  Journal                  = {{IEEE/ACM} Trans. Netw.},
  Year                     = {2007},

  Month                    = {Jun.},
  Number                   = {3},
  Pages                    = {574--587},
  Volume                   = {15}
}

@InProceedings{wang2006efficient,
  Title                    = {Efficient interference-aware TDMA link scheduling for static wireless networks},
  Author                   = {Wang, Weizhao and Wang, Yu and Li, Xiang-Yang and Song, Wen-Zhan and Frieder, Ophir},
  Booktitle                = {Proc. {ACM} international conference on Mobile computing and networking (MobiCom)},
  Year                     = {2006},
  Pages                    = {262--273}
}

@Article{weber2007transmission,
  Title                    = {Transmission capacity of wireless ad hoc networks with successive interference cancellation},
  Author                   = {Weber, Steven P and Andrews, Jeffrey G and Yang, Xiangying and De Veciana, Gustavo},
  Journal                  = {{IEEE} Trans. Inform. Theory},
  Year                     = {2007},

  Month                    = {Aug.},
  Number                   = {8},
  Pages                    = {2799--2814},
  Volume                   = {53}
}

@Article{weber2005transmission,
  Title                    = {Transmission capacity of wireless ad hoc networks with outage constraints},
  Author                   = {Weber, Steven P and Yang, Xiangying and Andrews, Jeffrey G and De Veciana, Gustavo},
  Journal                  = {{IEEE} Trans. Inform. Theory},
  Year                     = {2005},

  Month                    = {Dec.},
  Number                   = {12},
  Pages                    = {4091--4102},
  Volume                   = {51}
}

@Article{wildman2014joint,
  Title                    = {On the Joint Impact of Beamwidth and Orientation Error on Throughput in Wireless Directional Poisson Networks},
  Author                   = {Wildman, Jeffrey and Nardelli, Pedro HJ and Latva-aho, Matti and Weber, Steven},
  Journal                  = {{IEEE} Trans. Wireless Commun.},
  Year                     = {2014},

  Month                    = {Dec.},
  Number                   = {12},
  Pages                    = {7072--7085},
  Volume                   = {13}
}

@InProceedings{xu2002effective,
  Title                    = {How effective is the {IEEE} 802.11 {RTS/CTS} handshake in ad hoc networks?},
  Author                   = {Xu, Kaixin and Gerla, Mario and Bae, Sang},
  Booktitle                = {Proc. {IEEE} Global Communications Conference (GLOBECOM)},
  Year                     = {2002},
  Pages                    = {72--76}
}

@Article{Xu2016,
  Title                    = {Distributed Association and Relaying with Fairness in MillimeterWaves Networks},
  Author                   = {Y. Xu and H. Shokri-Ghadikolaei and C. Fischione},
  Journal                  = {{IEEE} Trans. Wireless Commun.},
  Year                     = {2016},

  Month                    = {Dec.},
  Number                   = {12},
  Pages                    = {7955--7970},
  Volume                   = {15}
}

@Article{Yu2016Distributed,
  Title                    = {Distributed Association and Relaying with Fairness in MillimeterWaves Networks},
  Author                   = {Y. Xu and H. Shokri-Ghadikolaei and C. Fischione},
  Journal                  = {{IEEE} Trans. Wireless Commun.},
  Year                     = {2016},

  Month                    = {Dec.},
  Number                   = {12},
  Pages                    = {7955--7970},
  Volume                   = {15}
}

@Article{Yang2003Delay,
  Title                    = {Delay Distributions of Slotted {ALOHA} and {CSMA}},
  Author                   = {Y. Yang and T.P. Yum},
  Journal                  = {{IEEE} Trans. Commun.},
  Year                     = {2003},

  Month                    = {Nov.},
  Number                   = {11},
  Pages                    = {1846--1857},
  Volume                   = {51}
}

@Article{ye2013user,
  Title                    = {User association for load balancing in heterogeneous cellular networks},
  Author                   = {Ye, Qiaoyang and Rong, Beiyu and Chen, Yudong and Al-Shalash, Mazin and Caramanis, Constantine and Andrews, Jeffrey G},
  Journal                  = {{IEEE} Trans. Wireless Commun.},
  Year                     = {2013},

  Month                    = {Jun.},
  Number                   = {6},
  Pages                    = {2706--2716},
  Volume                   = {12}
}

@Article{ye2004medium,
  Title                    = {Medium access control with coordinated adaptive sleeping for wireless sensor networks},
  Author                   = {Ye, Wei and Heidemann, John and Estrin, Deborah},
  Journal                  = {{IEEE/ACM} Trans. Netw.},
  Year                     = {2004},

  Month                    = {Jun.},
  Number                   = {3},
  Pages                    = {493--506},
  Volume                   = {12}
}

@Article{yi2014topological,
  Title                    = {Topological interference management with transmitter cooperation},
  Author                   = {Yi, Xinping and Gesbert, David},
  Journal                  = {{IEEE} Trans. Wireless Commun.},
  Year                     = {2015},

  Month                    = {Nov.},
  Number                   = {11},
  Pages                    = {6107--6130},
  Volume                   = {61}
}

@article{karakus2019redundancy,
  title={Redundancy Techniques for Straggler Mitigation in Distributed Optimization and Learning.},
  author={Karakus, Can and Sun, Yifan and Diggavi, Suhas N and Yin, Wotao},
  journal={Journal of Machine Learning Research},
  volume={20},
  number={72},
  pages={1--47},
  year={2019}
}

@ARTICLE{7736044,
author={M. {Ivanov} and F. {Brännström} and A. {Graell i Amat} and P. {Popovski}},
journal={IEEE Transactions on Communications},
title={Broadcast Coded Slotted-{ALOHA}: A Finite Frame Length Analysis},
year={2017},
volume={65},
number={2},
pages={651-662},
month={Feb.},}

@Article{Yu_HybridAM_16,
  Title                    = {Alternating Minimization Algorithms for Hybrid Precoding in Millimeter Wave {MIMO} Systems},
  Author                   = {Xianghao Yu and Juei{-}Chin Shen and Jun Zhang and Khaled Ben Letaief},
  Journal                  = {IEEE Journal of Selected Topics in Signal Processing},
  Year                     = {2016},
  Month                    = {Apr.},
  Number                   = {3},
  Pages                    = {485--500},
  Volume                   = {10}
}

@Article{zhang2015full,
  Title                    = {Full duplex techniques for {5G} networks: self-interference cancellation, protocol design, and relay selection},
  Author                   = {Zhang, Zhongshan and Chai, Xiaomeng and Long, Keping and Vasilakos, Athanasios V and Hanzo, Lajos},
  Journal                  = {{IEEE} Commun. Mag.},
  Year                     = {2015},

  Month                    = {May},
  Number                   = {5},
  Pages                    = {128--137},
  Volume                   = {53}
}

@InProceedings{zhao201328,
  Title                    = {28 {GHz} millimeter wave cellular communication measurements for reflection and penetration loss in and around buildings in {New York City}},
  Author                   = {Zhao, Hang and Mayzus, Rimma and Sun, Shu and Samimi, Mathew and Schulz, Jocelyn K and Azar, Yaniv and Wang, Kevin and Wong, George N and Gutierrez, Felix and Rappaport, Theodore S},
  Booktitle                = {Proc. {IEEE} International Conference on Communications (ICC)},
  Year                     = {2013},
  Pages                    = {5163--5167}
}

@InProceedings{Zhao201328Ghz,
  Title                    = {28 {GHz} millimeter wave cellular communication measurements for reflection and penetration loss in and around buildings in {New York} city},
  Author                   = {H. Zhao and R. Mayzus and S. Sun and M. Samimi and J. K. Schulz and Y. Azar and K. Wang and G. N. Wong and F. Gutierrez and T. S. Rappaport},
  Booktitle                = {Proc. {IEEE} International Conference on Communications (ICC)},
  Year                     = {2013},
  Pages                    = {5163--5167}
}

@Article{Zheng2015Gbs,
  Title                    = {{10 Gb/s} {HetSNets} with Millimeter-Wave Communications: {A}ccess and Networking -- Challenges and Protocols},
  Author                   = {K. Zheng and L. Zhao and J. Mei and M. Dohler and W. Xiang and Y. Peng},
  Journal                  = {{IEEE} Commun. Mag.},
  Year                     = {2015},

  Month                    = {Jan.},
  Number                   = {1},
  Pages                    = {222--231},
  Volume                   = {53},

  File                     = {#F#}
}

@book{tse2005fundamentals,
  title={Fundamentals of wireless communication},
  author={Tse, David and Viswanath, Pramod},
  year={2005},
  publisher={Cambridge University Press}
}

@ARTICLE{Ghauch_SRMax_17,
author={H. Ghauch and T. Kim and M. Bengtsson and M. Skoglund},
journal={{IEEE} J. Sel. Areas Commun.},
title={Sum-Rate Maximization in Sub-28-{GHz} Millimeter-Wave {MIMO} Interfering Networks},
year={2017},
volume={35},
number={7},
pages={1649-1662},
ISSN={0733-8716},
month={Jul.},}

@book{bertsekas2004data,
  title={Data networks, second edition},
  author={Bertsekas, Dimitri P and Gallager, Robert G and Humblet, Pierre},
  volume={2},
  year={2004},
  publisher={Prentice-Hall International New Jersey}
}

@book{Berstakas_nonlinear_99,
	Author = {Bertsekas, D.P.},
	Date-Added = {2016-05-05 14:38:46 +0000},
	Date-Modified = {2016-05-05 14:38:46 +0000},
	Edition = {2},
	Publisher = {Athena Scientific},
	Title = {Nonlinear Programming},
	Year = 1999}

@article{elbatt2004joint,
  title={Joint scheduling and power control for wireless ad hoc networks},
  author={El Batt, Tamer and Ephremides, Anthony},
  journal={IEEE Trans. Wireless Commun.},
  volume={3},
  number={1},
  month={Jan.},
  pages={74--85},
  year={2004},
}

@Article{zheng2003diversity,
  Title                    = {Diversity and multiplexing: {A} fundamental tradeoff in multiple-antenna channels},
  Author                   = {Zheng, Lizhong and Tse, David NC},
  Journal                  = {{IEEE} Trans. Inf. Theory},
  Year                     = {2003},

  Month                    = {May},
  Number                   = {5},
  Pages                    = {1073--1096},
  Volume                   = {49}
}

@Article{Xia2015Practical,
  Title                    = {Practical Conflict Graphs in the Wild},
  Author                   = {Xia Zhou and Zengbin Zhang and Gang Wang and Xiaoxiao Yu and Ben Y. Zhao and Haitao Zheng},
  Journal                  = {{IEEE/ACM} Trans. Netw.},
  Year                     = {2015},

  Month                    = {Jun.},
  Number                   = {3},
  Volume                   = {23},

  File                     = {#F#}
}

@InProceedings{WiGig,
  Title                    = {Wireless {G}igabit {A}lliance. [Online]. {A}vailable: http://wirelessgigabitalliance.org/}
}

@InProceedings{802_11ad,
  Title                    = {{IEEE} 802.11ad. {P}art 11: {W}ireless {LAN} Medium Access Control ({MAC}) and Physical Layer ({PHY}) Specifications - Amendment 3: {E}nhancements for Very High Throughput in the 60 {GHz} Band},
  Year                     = {2012},
  Month                    = {Dec.}
}

@InProceedings{802_15_3c,
  Title                    = {{IEEE} 802.15.3c {P}art 15.3: {W}ireless Medium Access Control ({MAC}) and Physical Layer ({PHY}) Specifications for High Rate Wireless Personal Area Networks ({WPANs}) Amendment 2: {M}illimeter-wave-based Alternative Physical Layer Extension},
  Year                     = {2009},
  Month                    = {Oct.}
}

@InProceedings{WirelessHD,
  Title                    = {Wireless{HD}: Wireless{HD} specification overview},
  Year                     = {2009}
}
@article{xiao2018distributed,
  title={Distributed optimization for energy-efficient fog computing in the Tactile Internet},
  author={Xiao, Yong and Krunz, Marwan},
  journal={IEEE Journal on Selected Areas in Communications},
  volume={36},
  number={11},
  pages={2390--2400},
  year={2018},
  publisher={IEEE}
}
@article{xiao2018distributed,
  title={Distributed optimization for energy-efficient fog computing in the tactile internet},
  author={Xiao, Yong and Krunz, Marwan},
  journal={IEEE Journal on Selected Areas in Communications},
  volume={36},
  number={11},
  pages={2390--2400},
  year={2018},
  publisher={IEEE}
}
@article{fan2018application,
  title={Application aware workload allocation for edge computing-based {IoT}},
  author={Fan, Qiang and Ansari, Nirwan},
  journal={IEEE Internet of Things Journal},
  volume={5},
  number={3},
  pages={2146--2153},
  year={2018},
  publisher={IEEE}
}

@Conference{Zhang:15,
  Title                    = {Spectrum Prediction and Channel Selection for Sensing-based Spectrum Sharing Scheme Using Online Learning Techniques},
  Author                   = {Z. Zhang and K. Zhang and F. Gao and S. Zhang},
  Booktitle                = {IEEE International Symposium on Personal, Indoor and Mobile Radio Communications (PIMRC)},
  Year                     = {2015},

  Owner                    = {gaborf},
  Timestamp                = {2018.05.08}
}
@article{elbamby2019wireless,
  title={Wireless Edge Computing with Latency and Reliability Guarantees},
  author={Elbamby, Mohammed S and Perfecto, Cristina and Liu, Chen-Feng and Park, Jihong and Samarakoon, Sumudu and Chen, Xianfu and Bennis, Mehdi},
  journal={arXiv preprint arXiv:1905.05316},
  year={2019}
}
@article{han2019convergence,
  title={Convergence of Edge Computing and Deep Learning: A Comprehensive Survey},
  author={Han, Yiwen and Wang, Xiaofei and Leung, Victor and Niyato, Dusit and Yan, Xueqiang and Chen, Xu},
  journal={arXiv preprint arXiv:1907.08349},
  year={2019}
}

@article{park2018wireless,
  title={Wireless network intelligence at the edge},
  author={Park, Jihong and Samarakoon, Sumudu and Bennis, Mehdi and Debbah, M{\'e}rouane},
  journal={Proc. {IEEE}},
  volume = {107},
  number = {11},
  pages = {2204--2239},
  month={Nov.},
  year = {2019},
}

@Conference{Forough:2019,
  Title                    = {Efficient Learning on High- dimensional Operational Data},
  Author                   = {F. S. Samani and H. Zhang and R. Stadler},
  Booktitle                = {15th IEEE International Conference on Network and Service Management (CNSM)},
  Year                     = {2019},

  Owner                    = {rolf},
  Timestamp                = {2019.05.08}
}


@article{lin2017deep,
  title={Deep gradient compression: Reducing the communication bandwidth for distributed training},
  author={Lin, Yujun and Han, Song and Mao, Huizi and Wang, Yu and Dally, William J},
  journal={arXiv preprint arXiv:1712.01887},
  year={2017}
}

@inproceedings{stich2018sparsified,
  title={Sparsified {SGD} with memory},
  author={Stich, Sebastian U and Cordonnier, Jean-Baptiste and Jaggi, Martin},
  booktitle={Advances in Neural Information Processing Systems},
  pages={4447--4458},
  year={2018}
}

@inproceedings{wangni2018gradient,
  title={Gradient sparsification for communication-efficient distributed optimization},
  author={Wangni, Jianqiao and Wang, Jialei and Liu, Ji and Zhang, Tong},
  booktitle={Advances in Neural Information Processing Systems},
  pages={1299--1309},
  year={2018}
}

@article{fan2019communication,
  title={Communication-Efficient Accurate Statistical Estimation},
  author={Fan, Jianqing and Guo, Yongyi and Wang, Kaizheng},
  journal={arXiv preprint arXiv:1906.04870},
  year={2019}
}

@article{yang2019energy,
  title={Energy Efficient Federated Learning Over Wireless Communication Networks},
  author={Yang, Zhaohui and Chen, Mingzhe and Saad, Walid and Hong, Choong Seon and Shikh-Bahaei, Mohammad},
  journal={arXiv preprint arXiv:1911.02417},
  year={2019}
}

@article{ziouva2002csma,
  title={{CSMA/CA} performance under high traffic conditions: {T}hroughput and delay analysis},
  author={Ziouva, Eustathia and Antonakopoulos, Theodore},
  journal={Computer communications},
  volume={25},
  number={3},
  pages={313--321},
  year={2002},
  publisher={Elsevier}
}

@article{smith2016cocoa,
  title={{CoCoA}: A general framework for communication-efficient distributed optimization},
  author = {Virginia Smith and Simone Forte and Chenxin Ma and Martin Tak{{\'a}}{\v{c}} and Michael I. Jordan and Martin Jaggi},
  journal={Journal of Machine Learning Research},
  volume = {18},
  number = {230},
  pages={1--49},
  year={2018}
}


@online{CSMA/CAlink,
  url = {https://people.cs.clemson.edu/~westall/851/802.11/802_CSMA_CA.pdf}
}

@inproceedings{mahmoudi_Journal,
  title={Is Co-design of Distributed Optimization and Communication Protocols Essential for Machine Learning over Networks?},
  author={Afsaneh Mahmoudi and Hossein S. Ghadikolaei and Carlo Fischione},
  Booktitle = {submitted to {IEEE} Transactions on Communications},
  year={2020}, url = {https://www.dropbox.com/sh/2r2wxrtnr6ogibq/AACI3gYGKeglCgyXlNZtZHlha?dl=0}
}


@article{chen2020convergence,
  title={Convergence Time Optimization for Federated Learning over Wireless Networks},
  author={Chen, Mingzhe and Poor, H Vincent and Saad, Walid and Cui, Shuguang},
  journal={arXiv preprint arXiv:2001.07845},
  year={2020}
}

%%%%%%%%% TPDS ----------------

@article{liu2020accelerating,
  title={Accelerating Federated Learning via Momentum Gradient Descent},
  author={Liu, Wei and Chen, Li and Chen, Yunfei and Zhang, Wenyi},
  journal={IEEE Transactions on Parallel and Distributed Systems},
  volume={31},
  number={8},
  pages={1754--1766},
  year={2020},
  publisher={IEEE}
}

@article{yuan2014communication,
  title={Communication-efficient decentralized event monitoring in wireless sensor networks},
  author={Yuan, Kun and Ling, Qing and Tian, Zhi},
  journal={IEEE Transactions on Parallel and Distributed Systems},
  volume={26},
  number={8},
  pages={2198--2207},
  year={2014},
  publisher={IEEE}
}

@article{yi2020efficient,
  title={Efficient Compute-Intensive Job Allocation in Data Centers via Deep Reinforcement Learning},
  author={Yi, Deliang and Zhou, Xin and Wen, Yonggang and Tan, Rui},
  journal={IEEE Transactions on Parallel and Distributed Systems},
  volume={31},
  number={6},
  pages={1474--1485},
  year={2020},
  publisher={IEEE}
}



@article{dass2018fast,
  title={Fast and communication-efficient algorithm for distributed support vector machine training},
  author={Dass, Jyotikrishna and Sarin, Vivek and Mahapatra, Rabi N},
  journal={IEEE Transactions on Parallel and Distributed Systems},
  volume={30},
  number={5},
  pages={1065--1076},
  year={2018},
  publisher={IEEE}
}


@article{peng2020lock,
  title={Lock-Free Parallelization for Variance-Reduced Stochastic Gradient Descent on Streaming Data},
  author={Peng, Yaqiong and Hao, Zhiyu and others},
  journal={IEEE Transactions on Parallel and Distributed Systems},
  year={2020},
  publisher={IEEE}
}

@article{di2018efficient,
  title={Efficient lossy compression for scientific data based on pointwise relative error bound},
  author={Di, Sheng and Tao, Dingwen and Liang, Xin and Cappello, Franck},
  journal={IEEE Transactions on Parallel and Distributed Systems},
  volume={30},
  number={2},
  pages={331--345},
  year={2018},
  publisher={IEEE}
}

@article{di2017optimization,
  title={Optimization of error-bounded lossy compression for hard-to-compress HPC data},
  author={Di, Sheng and Cappello, Franck},
  journal={IEEE transactions on parallel and distributed systems},
  volume={29},
  number={1},
  pages={129--143},
  year={2017},
  publisher={IEEE}
}



@inproceedings{xu2019signprox,
  title={Signprox: One-bit proximal algorithm for nonconvex stochastic optimization},
  author={Xu, Xiaojian and Kamilov, Ulugbek S},
  booktitle={ICASSP 2019-2019 IEEE International Conference on Acoustics, Speech and Signal Processing (ICASSP)},
  pages={7800--7804},
  year={2019},
  organization={IEEE}
}


@article{de2018high,
  title={High-accuracy low-precision training},
  author={De Sa, Christopher and Leszczynski, Megan and Zhang, Jian and Marzoev, Alana and Aberger, Christopher R and Olukotun, Kunle and R{\'e}, Christopher},
  journal={arXiv preprint arXiv:1803.03383},
  year={2018}
}


@inproceedings{stich2018sparsified,
  title={Sparsified SGD with memory},
  author={Stich, Sebastian U and Cordonnier, Jean-Baptiste and Jaggi, Martin},
  booktitle={Advances in Neural Information Processing Systems},
  pages={4447--4458},
  year={2018}
}


@inproceedings{magnusson2019maintaining,
  title={On maintaining linear convergence of distributed learning and optimization under limited communication},
  author={Magn{\'u}sson, Sindri and Shokri-Ghadikolaei, Hossein and Li, Na},
  booktitle={2019 53rd Asilomar Conference on Signals, Systems, and Computers},
  pages={432--436},
  year={2019},
  organization={IEEE}
}



@article{karimireddy2019error,
  title={Error feedback fixes signsgd and other gradient compression schemes},
  author={Karimireddy, Sai Praneeth and Rebjock, Quentin and Stich, Sebastian U and Jaggi, Martin},
  journal={arXiv preprint arXiv:1901.09847},
  year={2019}
}


@inproceedings{chen2018lag,
  title={{LAG}: Lazily aggregated gradient for communication-efficient distributed learning},
  author={Chen, Tianyi and Giannakis, Georgios and Sun, Tao and Yin, Wotao},
  booktitle={Advances in Neural Information Processing Systems},
  pages={5050--5060},
  year={2018}
}


@inproceedings{sun2019communication,
  title={Communication-efficient distributed learning via lazily aggregated quantized gradients},
  author={Sun, Jun and Chen, Tianyi and Giannakis, Georgios and Yang, Zaiyue},
  booktitle={Advances in Neural Information Processing Systems},
  pages={3370--3380},
  year={2019}
}


%@inproceedings{hsieh2017gaia,
 % title={Gaia: Geo-distributed machine learning approaching $\{$LAN$\}$ speeds},
 % author={Hsieh, Kevin and Harlap, Aaron and Vijaykumar, Nandita and Konomis, Dimitris and Ganger, Gregory R and Gibbons, Phillip B and Mutlu, Onur},
 % booktitle={14th $\{$USENIX$\}$ Symposium on Networked Systems Design and Implementation ($\{$NSDI$\}$ 17)},
 % pages={629--647},
 % year={2017}
%}
@inproceedings{hsieh2017gaia,
  title={Gaia: Geo-distributed machine learning approaching speeds},
  author={Hsieh, Kevin and Harlap, Aaron and Vijaykumar, Nandita and Konomis, Dimitris and Ganger, Gregory R and Gibbons, Phillip B and Mutlu, Onur},
  booktitle={14th Symposium on Networked Systems Design and Implementation},
  pages={629--647},
  year={2017}
}


@article{wang2019adaptive,
  title={Adaptive federated learning in resource constrained edge computing systems},
  author={Wang, Shiqiang and Tuor, Tiffany and Salonidis, Theodoros and Leung, Kin K and Makaya, Christian and He, Ting and Chan, Kevin},
  journal={IEEE Journal on Selected Areas in Communications},
  volume={37},
  number={6},
  pages={1205--1221},
  year={2019},
  publisher={IEEE}
}



@inproceedings{tandon2017gradient,
  title={Gradient coding: Avoiding stragglers in distributed learning},
  author={Tandon, Rashish and Lei, Qi and Dimakis, Alexandros G and Karampatziakis, Nikos},
  booktitle={International Conference on Machine Learning},
  pages={3368--3376},
  year={2017}
}


@article{reisizadeh2019coded,
  title={Coded computation over heterogeneous clusters},
  author={Reisizadeh, Amirhossein and Prakash, Saurav and Pedarsani, Ramtin and Avestimehr, Amir Salman},
  journal={IEEE Transactions on Information Theory},
  volume={65},
  number={7},
  pages={4227--4242},
  year={2019},
  publisher={IEEE}
}


@inproceedings{ozfatura2019speeding,
  title={Speeding up distributed gradient descent by utilizing non-persistent stragglers},
  author={Ozfatura, Emre and G{\"u}nd{\"u}z, Deniz and Ulukus, Sennur},
  booktitle={2019 IEEE International Symposium on Information Theory (ISIT)},
  pages={2729--2733},
  year={2019},
  organization={IEEE}
}


@inproceedings{yu2019lagrange,
  title={Lagrange coded computing: Optimal design for resiliency, security, and privacy},
  author={Yu, Qian and Li, Songze and Raviv, Netanel and Kalan, Seyed Mohammadreza Mousavi and Soltanolkotabi, Mahdi and Avestimehr, Salman A},
  booktitle={The 22nd International Conference on Artificial Intelligence and Statistics},
  pages={1215--1225},
  year={2019}
}

@inproceedings{narahari1994matching,
  title={Matching and scheduling in a generalized optimal selection theory},
  author={Narahari, Bhagirath and Youssef, Abdou and Choi, Hyeong-Ah},
  booktitle={Proceedings Heterogeneous Computing Workshop},
  pages={3--8},
  year={1994},
  organization={IEEE}
}


@article{hoefler2014overview,
  title={An overview of topology mapping algorithms and techniques in high-performance computing},
  author={Hoefler, Torsten and Jeannot, Emmanuel and Mercier, Guillaume},
  journal={High-Performance Computing on Complex Environments},
  volume={96},
  pages={75},
  year={2014},
  publisher={Wiley Online Library}
}


@article{topcuoglu2002performance,
  title={Performance-effective and low-complexity task scheduling for heterogeneous computing},
  author={Topcuoglu, Haluk and Hariri, Salim and Wu, Min-you},
  journal={IEEE transactions on parallel and distributed systems},
  volume={13},
  number={3},
  pages={260--274},
  year={2002},
  publisher={IEEE}
}


@article{mao2017survey,
  title={A survey on mobile edge computing: The communication perspective},
  author={Mao, Yuyi and You, Changsheng and Zhang, Jun and Huang, Kaibin and Letaief, Khaled B},
  journal={IEEE Communications Surveys \& Tutorials},
  volume={19},
  number={4},
  pages={2322--2358},
  year={2017},
  publisher={IEEE}
}



@article{li2019online,
  title={Online Placement and Scaling of Geo-Distributed Machine Learning Jobs via Volume-Discounting Brokerage},
  author={Li, Xiaotong and Zhou, Ruiting and Jiao, Lei and Wu, Chuan and Deng, Yuhang and Li, Zongpeng},
  journal={IEEE Transactions on Parallel and Distributed Systems},
  volume={31},
  number={4},
  pages={948--966},
  year={2019},
  publisher={IEEE}
}



@article{zhou2019privacy,
  title={Privacy regulation aware process mapping in geo-distributed cloud data centers},
  author={Zhou, Amelie Chi and Xiao, Yao and Gong, Yifan and He, Bingsheng and Zhai, Jidong and Mao, Rui},
  journal={IEEE Transactions on Parallel and Distributed Systems},
  volume={30},
  number={8},
  pages={1872--1888},
  year={2019},
  publisher={IEEE}
}


@inproceedings{chu2007map,
  title={Map-reduce for machine learning on multicore},
  author={Chu, Cheng-Tao and Kim, Sang K and Lin, Yi-An and Yu, YuanYuan and Bradski, Gary and Olukotun, Kunle and Ng, Andrew Y},
  booktitle={Advances in neural information processing systems},
  pages={281--288},
  year={2007}
}


@article{low2012distributed,
  title={Distributed graphlab: A framework for machine learning in the cloud},
  author={Low, Yucheng and Gonzalez, Joseph and Kyrola, Aapo and Bickson, Danny and Guestrin, Carlos and Hellerstein, Joseph M},
  journal={arXiv preprint arXiv:1204.6078},
  year={2012}
}


@inproceedings{abadi2016tensorflow,
  title={Tensorflow: A system for large-scale machine learning},
  author={Abadi, Mart{\'\i}n and Barham, Paul and Chen, Jianmin and Chen, Zhifeng and Davis, Andy and Dean, Jeffrey and Devin, Matthieu and Ghemawat, Sanjay and Irving, Geoffrey and Isard, Michael and others},
  booktitle={12th $\{$USENIX$\}$ symposium on operating systems design and implementation ($\{$OSDI$\}$ 16)},
  pages={265--283},
  year={2016}
}

@article{bernstein2018signsgd,
  title={signSGD: Compressed optimisation for non-convex problems},
  author={Bernstein, Jeremy and Wang, Yu-Xiang and Azizzadenesheli, Kamyar and Anandkumar, Anima},
  journal={arXiv preprint arXiv:1802.04434},
  year={2018}
}


@inproceedings{xu2019signprox,
  title={Signprox: One-bit proximal algorithm for nonconvex stochastic optimization},
  author={Xu, Xiaojian and Kamilov, Ulugbek S},
  booktitle={ICASSP 2019-2019 IEEE International Conference on Acoustics, Speech and Signal Processing (ICASSP)},
  pages={7800--7804},
  year={2019},
  organization={IEEE}
}

@article{miller1971minimizing,
  title={On minimizing nonseparable functions defined on the integers with an inventory application},
  author={Miller, Bruce L},
  journal={SIAM Journal on Applied Mathematics},
  volume={21},
  number={1},
  pages={166--185},
  year={1971},
  publisher={SIAM}
}
%%%------ Cognitive radio networks---
@ARTICLE{8542764,  author={O. {Simeone}},  journal={IEEE Transactions on Cognitive Communications and Networking},   title={A Very Brief Introduction to Machine Learning With Applications to Communication Systems},   year={2018},  volume={4},  number={4},  pages={648-664},  doi={10.1109/TCCN.2018.2881442}}

@ARTICLE{8054694,  author={T. {O’Shea} and J. {Hoydis}},  journal={IEEE Transactions on Cognitive Communications and Networking},   title={An Introduction to Deep Learning for the Physical Layer},   year={2017},  volume={3},  number={4},  pages={563-575},  doi={10.1109/TCCN.2017.2758370}}

@ARTICLE{9107235,  author={D. {Liu} and G. {Zhu} and J. {Zhang} and K. {Huang}},  journal={IEEE Transactions on Cognitive Communications and Networking},   title={Data-Importance Aware User Scheduling for Communication-Efficient Edge Machine Learning},   year={2020},  volume={},  number={},  pages={1-1},  doi={10.1109/TCCN.2020.2999606}}

%%%--------------------------------

@ARTICLE{8861393,  author={X. {Cao} and L. {Lai}},  journal={IEEE Transactions on Signal Processing},   title={Distributed Gradient Descent Algorithm Robust to an Arbitrary Number of Byzantine Attackers},   year={2019},  volume={67},  number={22},  pages={5850-5864},  doi={10.1109/TSP.2019.2946020}}

@ARTICLE{9264742,  author={Z. {Yang} and M. {Chen} and W. {Saad} and C. S. {Hong} and M. {Shikh-Bahaei}},  journal={IEEE Transactions on Wireless Communications},   title={Energy Efficient Federated Learning Over Wireless Communication Networks},   year={2020},  volume={},  number={},  pages={1-1},  doi={10.1109/TWC.2020.3037554}}


@ARTICLE{9127160,  author={S. {Luo} and X. {Chen} and Q. {Wu} and Z. {Zhou} and S. {Yu}},  journal={IEEE Transactions on Wireless Communications},   title={{HFEL}: Joint Edge Association and Resource Allocation for Cost-Efficient {H}ierarchical {F}ederated {E}dge {L}earning},   year={2020},  volume={19},  number={10},  pages={6535-6548},  doi={10.1109/TWC.2020.3003744}}

@ARTICLE{1094462,  author={Rubin, I.},  journal={IEEE Transactions on Communications},   title={Message Delays in FDMA and TDMA Communication Channels},   year={1979},  volume={27},  number={5},  pages={769-777},  doi={10.1109/TCOM.1979.1094462}}

@ARTICLE{1056095,  author={Rubin, I.},  journal={IEEE Transactions on Information Theory},   title={Access-control disciplines for multi-access communication channels: Reservation and TDMA schemes},   year={1979},  volume={25},  number={5},  pages={516-536},  doi={10.1109/TIT.1979.1056095}}



@article{nguyen2020efficient,
  title={Efficient Federated Learning Algorithm for Resource Allocation in Wireless {I}o{T} Networks},
  author={Nguyen, Van Dinh and Sharma, Shree Krishna and Vu, Thang Xuan and Chatzinotas, Symeon and Ottersten, Bj{\"o}rn},
  journal={IEEE Internet of Things Journal},
  year={2020},
  publisher={Institute of Electrical and Electronics Engineers}
}

@article{li2019convergence,
  title={On the convergence of fedavg on non-iid data},
  author={Li, Xiang and Huang, Kaixuan and Yang, Wenhao and Wang, Shusen and Zhang, Zhihua},
  journal={arXiv preprint arXiv:1907.02189},
  year={2019}
}

@ARTICLE{9563954,  author={Thompson, Neil C. and Greenewald, Kristjan and Lee, Keeheon and Manso, Gabriel F.},  journal={IEEE Spectrum},   title={Deep Learning's Diminishing Returns: The Cost of Improvement is Becoming Unsustainable},   year={2021},  volume={58},  number={10},  pages={50-55},  doi={10.1109/MSPEC.2021.9563954}}

@inproceedings{balatsoukas2019deep,
  title={Deep unfolding for communications systems: A survey and some new directions},
  author={Balatsoukas-Stimming, Alexios and Studer, Christoph},
  booktitle={2019 IEEE International Workshop on Signal Processing Systems (SiPS)},
  pages={266--271},
  year={2019},
  organization={IEEE}
}

@ARTICLE{7786995,  author={},  journal={IEEE Std 802.11-2016 (Revision of IEEE Std 802.11-2012)},   title={IEEE standard for information technology—telecommunications and information exchange between systems local and metropolitan area networks—specific requirements - Part 11: Wireless LAN Medium Access Control (MAC) and Physical Layer (PHY) specifications},   year={2016},  volume={},  number={},  pages={1-3534},  doi={10.1109/IEEESTD.2016.7786995}}


@INPROCEEDINGS{8422767,  author={Bankov, Dmitry and Didenko, Andre and Khorov, Evgeny and Lyakhov, Andrey},  booktitle={2018 IEEE International Conference on Communications (ICC)},   title={{OFDMA} Uplink Scheduling in {IEEE} 802.11ax Networks},   year={2018},  volume={},  number={},  pages={1-6},  doi={10.1109/ICC.2018.8422767}}



@ARTICLE{8889996,  author={Sattler, Felix and Wiedemann, Simon and Müller, Klaus-Robert and Samek, Wojciech},  journal={IEEE Transactions on Neural Networks and Learning Systems},   title={Robust and Communication-Efficient {F}ederated {L}earning From Non-i.i.d. Data},   year={2020},  volume={31},  number={9},  pages={3400-3413},  doi={10.1109/TNNLS.2019.2944481}}


@article{konevcny2016federated,
  title={Federated learning: Strategies for improving communication efficiency},
  author={Kone{\v{c}}n{\`y}, Jakub and McMahan, H Brendan and Yu, Felix X and Richt{\'a}rik, Peter and Suresh, Ananda Theertha and Bacon, Dave},
  journal={arXiv preprint arXiv:1610.05492},
  year={2016}
}

@ARTICLE{1245995,  author={Yang Yang and Yum, T.-S.P.},  journal={IEEE Transactions on Communications},   title={Delay distributions of slotted {ALOHA{ and {CSMA},   year={2003},  volume={51},  number={11},  pages={1846-1857},  doi={10.1109/TCOMM.2003.819201}}

@ARTICLE{8425988,  author={Malandra, Filippo and Sansò, Brunilde},  journal={IEEE Transactions on Wireless Communications},   title={A Markov-Modulated End-to-End Delay Analysis of Large-Scale {RF{ Mesh Networks With Time-Slotted {ALOHA} and {FHSS} for Smart Grid Applications},   year={2018},  volume={17},  number={11},  pages={7116-7127},  doi={10.1109/TWC.2018.2860965}}

@ARTICLE{4155680,  author={Casini, Enrico and De Gaudenzi, Riccardo and Del Rio Herrero, Oscar},  journal={IEEE Transactions on Wireless Communications},   title={Contention Resolution Diversity Slotted ALOHA (CRDSA): An Enhanced Random Access Schemefor Satellite Access Packet Networks},   year={2007},  volume={6},  number={4},  pages={1408-1419},  doi={10.1109/TWC.2007.348337}}

@book{DBLP:books/daglib/0022091,
  author    = {Igor Griva and
               Stephen G. Nash and
               Ariela Sofer},
  title     = {Linear and Nonlinear Optimization {(2.} ed.)},
  publisher = {{SIAM}},
  year      = {2008},
  isbn      = {978-0-89871-661-0},
  timestamp = {Wed, 16 Mar 2011 21:36:12 +0100},
  biburl    = {https://dblp.org/rec/books/daglib/0022091.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@ARTICLE{8086180,  author={Hoang, Tuong Duc and Bao Le, Long},  journal={IEEE Transactions on Wireless Communications},   title={Joint Prioritized Scheduling and Resource Allocation for {OFDMA}-Based Wireless Networks},   year={2018},  volume={17},  number={1},  pages={310-323},  doi={10.1109/TWC.2017.2765309}}

%%%%%%%%%%%%%%%% NEW work %%%%%%%%%%%%%%%%%
@article{li2020talk,
  title={To Talk or to Work: Flexible Communication Compression for Energy Efficient Federated Learning over Heterogeneous Mobile Edge Devices},
  author={Li, Liang and Shi, Dian and Hou, Ronghui and Li, Hui and Pan, Miao and Han, Zhu},
  journal={arXiv preprint arXiv:2012.11804},
  year={2020}
}

==> MetaFiles/packages_new.tex <==

% \usepackage[T1]{fontenc}
% \usepackage[font=sf]
\usepackage[T1]{fontenc}
\usepackage[scaled]{helvet}
\usepackage[final]{pdfpages}
\usepackage[T1]{fontenc}
\usepackage{pgfplots}
\usepackage{upgreek}
%\usepackage{dutchcal}
\usepackage{textcomp}
\usepackage{algorithm2e}
\SetNlSty{normal}{}{:}
\usepackage{algorithmic}
\usepackage{lmodern}
% \usepackage[latin1]{inputenc}
\usepackage[swedish, english]{babel}
\usepackage{graphics}
\usepackage{amssymb}
\usepackage{amsmath,amssymb,amsfonts}
\usepackage{mathtools}
\usepackage{tikz}
\usepackage{siunitx}
\usepackage[american,cuteinductors,smartlabels]{circuitikz}
\usepgfplotslibrary{polar}
\usepackage{ellipsis}
\usetikzlibrary{calc}
\usetikzlibrary{decorations.pathreplacing,decorations.markings,shapes.geometric}
\usepackage{amsthm}
\newtheorem{thm}{Theorem}
\newtheorem{lem}{Lemma}
\newtheorem{prop}[thm]{Proposition}
\newtheorem{cor}{Corollary}
\newtheorem{defn}{Definition}[section]
\newtheorem{conj}{Conjecture}[section]
\newtheorem{exmp}{Example}[section]
\newtheorem{rem}{Remark}

% \ctikzset{bipoles/thickness=1}
% \ctikzset{bipoles/length=0.8cm}
% \ctikzset{bipoles/diode/height=.375}
% \ctikzset{bipoles/diode/width=.3}
% \ctikzset{tripoles/thyristor/height=.8}
% \ctikzset{tripoles/thyristor/width=1}
% \ctikzset{bipoles/vsourceam/height/.initial=.7}
% \ctikzset{bipoles/vsourceam/width/.initial=.7}
% \tikzstyle{every node}=[font=\small]
% \tikzstyle{every path}=[line width=0.8pt,line cap=round,line join=round]
\usepackage{tikz-layers}
\usetikzlibrary{shapes}
\usepackage{siunitx}
\def\BibTeX{{\rm B\kern-.05em{\sc i\kern-.025em b}\kern-.08em
		T\kern-.1667em\lower.7ex\hbox{E}\kern-.125emX}}
\usetikzlibrary{trees}
\usepackage{circuitikz}
\usetikzlibrary{snakes,arrows,shapes}
\usetikzlibrary{calc,patterns,arrows,shapes.arrows,intersections}
\usetikzlibrary{arrows}
\usetikzlibrary{positioning,chains,fit,shapes,calc}
\usetikzlibrary{positioning}
\usetikzlibrary{decorations.pathmorphing}
\usetikzlibrary{decorations.markings}
\usetikzlibrary{decorations}
\usetikzlibrary{decorations.text}
\usetikzlibrary{decorations.pathmorphing}
\usetikzlibrary{shapes.misc, positioning}
\usepackage[hyphens]{url}
\usepackage[hidelinks]{hyperref}					% Clickable links
\hypersetup{breaklinks=true}
\usepackage{amsmath}
\usepackage{graphicx} 
\usepackage{caption}
% \usepackage{subcaption}
\usepackage{color} 
\usepackage{transparent} 
\usepackage{bm} % bold math
\usepackage{bbm}
\usepackage{fmtcount}
\usepackage{booktabs}
\usepackage{multirow}
\usepackage{url}
\usepackage{cite}
\usepackage[singlelinecheck=off]{caption}
\usepackage{stackengine}
\def\delequal{\mathrel{\ensurestackMath{\stackon[1pt]{=}{\scriptstyle\Delta}}}}
\usepackage{optidef}
\DeclareMathOperator*{\minimize}{minimize}
\DeclareMathOperator*{\maximize}{maximize}

\hypersetup{colorlinks = false, urlcolor=black}
\usepackage[caption=false]{subfig}
\usepackage[absolute,overlay]{textpos}

\usepackage[nopostdot,  style=super, nonumberlist, toc]{glossaries}
% \usepackage{glossaries}
\makeglossaries








% *** MATH PACKAGES ***
% \usepackage{amsmath}
% \usepackage{bm}
\usepackage[cmintegrals]{newtxmath}
\usepackage{afterpage}
% \usepackage{setspace}
% \usepackage{filecontents}

\usepackage{hyperref}
\usepackage{cleveref}
\hypersetup{
    colorlinks=false,
    linkcolor=blue,
    filecolor=magenta,      
    urlcolor=cyan,
    pdftitle={Overleaf Example},
    pdfpagemode=FullScreen,
    }
\def\delequal{\mathrel{\ensurestackMath{\stackon[1pt]{=}{\scriptstyle\Delta}}}}
\def\BibTeX{{\rm B\kern-.05em{\sc i\kern-.025em b}\kern-.08em
    T\kern-.1667em\lower.7ex\hbox{E}\kern-.125emX}}

  \captionsetup{size=small,
    %justification=centering, %% not needed
    skip=5pt, position = bottom}





